Fractal Rosette: A Stable Space-Ground Network Structure in Mega-Constellation

We present F-Rosette, a stable space-ground network structure for low-earth orbit (LEO) satellite mega-constellations at scale. Due to the dynamic many-to-many space-ground mapping in high mobility, existing LEO mega-constellations with IP protocol stack suffer from frequent user IP address changes (every 133~510s per user) and network routing re-convergence (<20% network usability). To provably stabilize the space-ground network under high mobility and many-to-many dynamics, F-Rosette adopts a recursive structure over the Rosette constellation, derives a hierarchical and time-invariant network address space from a new geographical coordinate system, and ensures efficient and stable routing via geographical-to-topological routing embedding without re-convergence. Our hardware-in-the-loop, trace-driven emulations validate F-Rosette's stability, near-optimal routing (<1.4% additional delays), and marginal overhead (<1% CPU, <2MB memory) for resource-constrained satellites.

==> Makefile <==
DOCUMENT=sigcomm19

default: $(DOCUMENT).pdf

$(DOCUMENT).toc: $(DOCUMENT).tex
	pdflatex --shell-escape $(DOCUMENT).tex

$(DOCUMENT).pdf: $(DOCUMENT).toc
	bibtex $(DOCUMENT)
	pdflatex --shell-escape $(DOCUMENT).tex
	pdflatex --shell-escape $(DOCUMENT).tex

#--------------------------------------------------
# $(DOCUMENT).ps: $(DOCUMENT).dvi
#     dvips -t letter -Ppdf -G0 -o $@ $<
#
# $(DOCUMENT).pdf: $(DOCUMENT).ps
#     cat $(DOCUMENT).ps | ps2pdf - > $(DOCUMENT).pdf
#--------------------------------------------------

all: $(DOCUMENT).pdf

clean:
	rm -rf *.aux $(DOCUMENT).log $(DOCUMENT).toc \
     $(DOCUMENT).bbl $(DOCUMENT).blg $(DOCUMENT).pdf \


==> abstract-v2.tex <==
\begin{abstract}

We present \name, a stable space-ground network structure for low-earth orbit (LEO) satellite mega-constellations at scale. 
Due to the dynamic many-to-many space-ground mapping in high mobility, existing LEO mega-constellations with IP protocol stack suffer from 
%dynamic many-to-many mapping between space and ground, which results in 
frequent user IP address changes (every 133--510s per user) and network routing re-convergence (thus $\leq$20\% network usability). 
%To solve these fundamental stability issues in the highly dynamic environment, 
To provably stabilize the space-ground network under high mobility and many-to-many dynamics,
%\name aims to bridge the gap between the network design in the virtual cyberspace and the mega-constellations in the physical world.
\name adopts a recursive structure over the Rosette constellation, 
derives a hierarchical and time-invariant network address space from a new geographical coordinate system, 
and ensures efficient and stable routing via geographical-to-topological routing embedding without re-convergence.
%and eliminates routing re-convergence with local geographical-to-topological routing embedding over its stable topology.
%To this end, \name stabilizes the space-ground network topology, addressing and routing in such a highly dynamic environment. 
%\name adopts a recursive structure with provably stable topology and devises hierarchical and time-invariant addressing for space and ground. 
%It eliminates the routing re-convergence, and enables geographical routing for terrestrial users by converting it to routing over stable topology. 
Our hardware-in-the-loop, trace-driven emulations validate \name's stability, near-optimal routing ($\leq$1.4\% additional delays), and marginal overhead (<1\% CPU,  <2MB memory) for resource-constrained satellites.

\end{abstract}






==> abstract.tex <==
\begin{abstract}

This paper presents \name, a new low-earth orbit (LEO) mega-constellation for stable, scalable, and efficient networking in space. 
Unlike state-of-the-art, \name's primary goal is to ensure stable and scalable network topology, addressing, and routing in the presence of massive fast-moving LEO satellite mobility and earth rotations, while still retain- ing full coverage and low latency. 
\name adopts a recursive network structure over LEO satellites on the earth-repeat orbits, divides the earth surface areas into a hierarchy of geographic cells across these orbits, and allocates a stable network address to terrestrial users and satellites based on geographical cells. 
\name supports efficient single-path routing with bounded latency, multi-path routing for high performance and fault tolerance, and on-demand incremental constellation expansion with fewer satellites. 
%Existing mega-constellations (such as Starlink, Kuiper, and Iridium) can be re-structured to \name to enjoy stable networking in space. 
Our trace-driven emulations over a satellite router testbed validate \name's advantages over existing mega-constellations.

\end{abstract}






==> address.tex <==
\subsection{Hierarchical Addressing in \name}
\label{sec:address}


\subsubsection{Logical addresses for satellites} 
\label{sec:address:sat}

%\wei{Two ways of constructing \name, with formula of node IDs, link IDs, and all equations.}

We assign each satellite $S$ in $\name_k$ with a hierarchical address \textsf{$s_0.s_1.s_2...s_{N-1}$} ($s_i=0,1,...,N-1, \forall i$).
Each digit $s_i$ represents the corresponding $\name_{i}$ structure that this satellite $S$ belongs to. 
%\lixin{Check if this address construction is consistent with your proposal.}


\subsubsection{Geographical addresses for terrestrial users}
\label{sec:address:ue}

%\name enables hierarchical and stable geographical cells divisions, thus facilitating {\em location-based} network addressing for terrestrial users. 


To facilitate the satellite networking for terrestrial users, \name decomposes the earth's spherical surface into a hierarchy of disjoint {\em geographical cells} and performs location-based routing for terrestrial users.
Figure \ref{fig:construction:cell} illustrates the cells in $\name_2$.
Each \name cell is a quadrilateral bounded by four satellite sub-point trajectories of \name's satellites. 
The \name cells exhibit three appealing features for satellite routing in space:

%We use the satellite sub-point trajectories of \name's satellites to divide the geographical cells on the earth surface. 
%As shown in Figure~\ref{XXX}\wei{Figure of satellite sub-points and cells}


\paragraphb{Time-invariant geographical cells:}
Recall that all satellites in \name are operated on the {\em repeat-earth} orbits ($\S$\ref{sec:construction}), which implies all satellite sub-point trajectories are {\em time-invariant}.
%Therefore, a \name cell that is bounded by four satellite sub-point trajectories covers a {\em fixed} earth surface area. 
Therefore, despite high satellite mobility and earth rotation, each \name cells's location, size, and coverage are {\em fixed} and do not vary over time.

\iffalse
\begin{thm}
The location and size of each geographic cell in $\name_k$ is time-invariant regardless of satellite movement and earth rotation. \jiayi{Add proof to appendix.}
\end{thm}
\fi

\begin{figure}[t]
\includegraphics[width=.5\columnwidth]{figures/hierarchical-cell-proof.pdf}
%\caption{Proof of Theorem~\ref{proof:hierarchy}.}
\caption{Hierarchical cells in \name.}
\label{fig:proof-hierarchy}
\end{figure}

\paragraphb{Hierarchical \name cells:}
\name's recursive and symmetric structure forms a hierarchy of cells.  
By recursively constructing \name, each cell in $\name_{k-1}$ will be uniformly divided into a group of sub-cells in $\name_{k}$.
%The following theorem unveils the concrete cell hierarchy (proved in Appendix~\ref{proof:hierarchy}: 
This hierarchy is exemplified in Figure~\ref{fig:proof-hierarchy} and illustrated by the following theorem (proved in Appendix~\ref{proof:hierarchy}): 

\begin{thm}
When constructing $\name_k$ from $\name_{k-1}$, each cell $\name_{k-1}$ will be divided in to $N^2$ disjoint sub-cells in $\name_k$.
\label{thm:hierarchy}
\end{thm}

We also have the total number of cells in a $\name_k$ as follows (proved in Appendix~\ref{proof:cells}): %\wei{Unify notations. Finish proof}:
\begin{lem}
A $\name_k$ has $[a(a-b-1)+2]N^{2k}$ disjoint cells, where $\frac{a}{b}=\frac{N^{k+1}-m}{N^k}$ with $a$ and $b$ being mutually prime.
\label{lem:cells}
\end{lem}

\paragraphb{Stable location-based routing across cells:}
Different from other geographic information systems for navigations (such as Google S2 \cite{google-s2} and Uber H3 \cite{uber-h3}), \name divides the geographical cells based on {\em satellite trajectories}, rather than traditional latitude/longitude or space-filling curves. 
In this way, the cell ID itself implies the satellite routing in \name.
We will elaborated on it in $\S$\ref{sec:routing:ue}.


\paragraphb{Hierarchical and stable address for terrestrial users:}
To this end, \name assigns geographical address to each terrestrial user based on the cell it resides it. 
A geographical cell in $\name_k$ is uniquely identified by $c_0.c_1...,.c_{N-1}$, where $c_0=0,1,...a(a-b-1)+1$ and $c_i=0,1,...,N^2-1 (i\neq0)$. 
Each digit $c_i$ represents the corresponding $\name_{i}$ cell identifier that this user belongs to. 
For each user in this cell, \name assigns its address as \textsf{net\_pref.cell\_ID.net\_suffix}, where \text{net\_pref} is the network prefix for heterogeneous inter-networking, \textsf{cell\_ID} is \name's hierarchical cell ID, and \textsf{net\_suffix} is per-user suffix that guarantees globally unique address inside each cell. 
In this way, the user address remains {\em invariant} unless (s)he moves to a new cell.
This address can be readily implemented with IPv6 address, segment routing (SRv6), or embedded into the address of other future Internet architecture such as NDN~\cite{zhang2014named,jacobson2009networking}, MobilityFirst \cite{mobilityfirst}, SCION \cite{zhang2011scion}, and XIA \cite{han2012xia}.
\yuanjie{Refine the writing here.}

%\yuanjie{Location-based routing here?}
\iffalse
\begin{compactitem}
\item Geographical cells;
\item Prefix for ground station
\item Suffix for duplicate address.
\end{compactitem}
\fi



==> architecture.tex <==
\section{The \name Mega-Constellation}
\label{sec:arch}


This section introduces the \name structure, basic properties, and addressing for satellites and terrestrial users. 

\input{rosette-primer}
\input{construction}
\input{properties}
\input{address}



==> background.tex <==
%\section{Networking in Space Today}
%\section{Mega Constellation for Space Networking}
\section{Networking in Space: A Primer}
\label{sec:back}

%\yuanjie{A design-space analysis to clarify \name's position: GEO, MEO, or LEO $\rightarrow$ coverage vs. networking $\rightarrow$ L2 or L3 (differentiate OneWeb) $\rightarrow$ Stable or dynamics (differentiate Starlink and Kuiper).}

\todo{Unify and simplify the notations. Define and minimize the necessary terms}

This section describes necessary background for the satellite mega-constellations today ($\S$\ref{sec:back:back}),
and explains why they suffer from network instability at scale ($\S$\ref{sec:challenge}). 

\input{sat-network}
%\input{use-case}
\input{challenge}



==> bib/eval-characteristics.tex <==
\subsection{Characteristics of \name}

==> challenge-v2.tex <==
%\subsection{Deficiencies of Mega-Constellations Today}
%\subsection{Unstable Mega-Constellations Today}
\subsection{Unstable Space-Ground Network Today}
\label{sec:challenge}

The LEO mega-constellations aim to enable ubiquitous low-latency network services for terrestrial users.
Since they are at the early stages of deployment, their network functions are still underway and tested at a tiny scale \cite{starlink-data-plan, starlink-isl-test,starlink-isl-test-2}.
Our trace-driven emulation projects that, {\em with high dynamics of relative motion between satellites and earth, existing mega-constellations with standard IP network will suffer from {unstable} services between space and ground}.

Compared to the MEO/GEO satellites, LEO satellites at much lower altitude (typically $\leq$2,000 km) exhibit high mobility\footnote{According to Kepler's third law, for all satellites of the earth, the ratio between their orbital altitude and period $(R_E+H_s)^3/T_s^2$ is a constant.} and relative motions.
Moreover, the earth's rotation further complicates the relative motions between satellites and terrestrial users.
Both result in frequent churns of the network links between satellites and terrestrial users and topology.
Such unstable topology causes two negative impacts for users and network:
%This results in frequent satellite network topology and inter-satellite link (ISL) changes.
%The unstable network services exhibit in three aspects:

\paragraphb{}

\paragraphb{Frequent IP address changes for terrestrial users:}
The classical IPv4/IPv6 address mostly adopts logical network addressing.
When a terrestrial user associates to a satellite, its IP address belongs to the subnet of the corresponding satellite network interface.
With rapid satellite motions, the terrestrial users served by one satellite have to frequently switch to new satellites (thus new network interfaces and address) to retain its Internet access. %(every 120--125s per user, and 1000--6000 IP address changes per second in Starlink). 
\del{As shown in Figure~\ref{fig:ip_change}, each user should change its logical IP address every 120--125s, and every 1000--6000 users per second should change their IP addresses as their serving satellites moves. }
%
\add{Based on the Gridded Population of the World Dataset published by NASA\cite{NASA2020}, we selected $10,011$ user points proportionally in the 20 most densely populated regions of the world. 
Based on the constellation trace information simulated by Starperf, each user selects the nearest satellite for access. 
Only if the selected access satellite no longer meets the access conditions, the same principle is used to select the connecting satellite. 
The results of user IP address changes under different constellation parameters within 3600s are shown in Figure~\ref{fig:user_ip_change}. 
Each user should change its logical IP address every 133--510s, and every 20--75 users per second among 10011 users should change their IP addresses as their serving homes moves.}
%\lixin{Update the number. Elaborate on the experiment methodology.}
Such frequent address changes will repetitively disrupt the TCP connections and upper-layer applications, thus negatively impacting the user experiences of satellite network services. 
\todo{Each satellite covers 100,000 users, its movement will cause significant IP changes among users.}

% \begin{figure}[t]
% \includegraphics[width=\columnwidth]{figures/user_ip_change.eps}
% \caption{Frequent changes of terrestrial users' IP addresses in state-of-the-art LEO mega-constellations.} %\lixin{Is IP change \wrt altitude a key point of this paper?}}
% \label{fig:user_ip_change}
% \end{figure}

\begin{figure}[t]
\subfloat[Interval between changes]{
\includegraphics[width=0.5\columnwidth]{figures/user_ip_change.eps}
\label{fig:user_ip_change}
}
\subfloat[IP changed users per second]{
\includegraphics[width=0.5\columnwidth]{figures/time_ip_change.eps}
\label{fig:timecdf_ip_change}
}
%\caption{Frequent reconfigurations of terrestrial users' IP addresses in state-of-the-art LEO mega-constellations.}
\caption{Projected ground users' IP address change frequency due to mobility of satellites in LEO mega-constellations.}
\label{fig:ip_change}
\end{figure}


\paragraphb{Frequent routing re-convergence for the network:}
If the classical Internet routing protocols were used in mega-constellations, the frequent topology change will result in frequent re-routing.
As an LEO satellite moves, it can only offer approximately \add{10-minute in Iridium, even less than 3-minute in Starlink} continuous service for each user before it leaves the coverage. 
Frequent routing re-convergence will further shorten the service time for this satellite and significantly lower the network usability.
Figure~\ref{fig:usability} illustrates the usability of mega-constellations using OSPF. %, a recently proposed LEO satellite inter-networking scheme.
\add{Six ground stations that locate in New York, Tokyo, Beijing, Hong Kong, Shanghai, and Singapore are selected. Each ground station selects the nearest satellite for access. 
When the satellite does not meet the access conditions, the next access satellite is selected based on the same selection principle. 
Based on the trace information of satellites under different scales simulated by Starperf, switching scenarios under multiple constellation scales within 100 minutes are generated. 
We used the Mininet network simulation tool to simulate the switching scenarios under different constellation scales, and obtained the network usability results as shown in Figure~\ref{fig:usability}.}
It shows that, all mega-constellations today suffer from $\leq20\%$ network usability even under small cosntellations. %\footnote{A common solution to scale link-state routing is to divide the mega-constellation into ASes. However, this unavoidably incurs tradeoff between scalability and routing efficiency (detouring). \yuanjie{To be polished.}}.\lixin{update the number}


\iffalse
The LEO mega-constellations today are primarily designed for enabling {\em full coverage} with low latency for the terrestrial users.
\del{Unfortunately, they fall short in enabling stable and efficient {\em inter-networking, addressing and routing}.}
\add{Since they are still at the early stages of deployment, they have not yet fully explored stable and efficient {\em inter-networking, addressing and routing}.}
With the high mobility of satellites and earth, networking with the existing mega-constellations suffers from three deficiencies of stability on the network and user sides:
\fi

\iffalse
\paragraphb{Unstable satellite network topology:}
Compared to the MEO/GEO satellites, LEO satellites at much lower altitude (typically $\leq$2,000 km) exhibit high mobility\footnote{According to Kepler's third law, for all satellites of the earth, the ratio between their orbital altitude and period $(R_E+H_s)^3/T_s^2$ is a constant.} and relative motions.
This results in frequent satellite network topology and inter-satellite link (ISL) changes.
It not only complicates the network routing in space, but also triggers repetitive re-convergence in link-state routing protocols and therefore significantly lowers the network usability.
%($\leq$10\% network availability for Starlink and Kuiper)\lixin{update the number}. 
Figure~\ref{fig:usability} illustrates the usability of mega-constellations using \textsf{motif}~\cite{bhattacherjee2019network}, a recently proposed LEO satellite inter-networking scheme.
\lixin{Methodology of the experiments}
It shows that, all mega-constellations today suffer from $\leq10\%$ network availability\footnote{A common solution to scale link-state routing is to divide the mega-constellation into ASes. However, this unavoidably incurs tradeoff between scalability and routing efficiency (detouring). \yuanjie{To be polished.}}.\lixin{update the number}

\lixin{For Iridium, show the empirical results of low network usable time. For Starlink, Kuiper and Telesat, show the convergence time \wrt number of satellites using \textsf{motif}.}
\fi

\begin{figure}[t]
\subfloat[Starlink]{
\includegraphics[width=0.5\columnwidth]{figures/starlink_usibility.eps}
\label{fig:starlink_usibility}
}
\subfloat[Kuiper]{
\includegraphics[width=0.5\columnwidth]{figures/kuiper_usibility.eps}
\label{fig:kuiper_usibility}
}
\caption{Projected network usability under routing re-convergence due to mobility of satellites in LEO mega-constellations.} %\lixin{(1) Why low availability (<80\%) when there are very few satellites? (2) Why very slow usability decrement as the constellation becomes larger? (3) How about motif in CoNEXT'19?}
\label{fig:usability}
\end{figure}

\iffalse
\paragraphb{Unstable user addressing:} 
The classical logical network addressing suffers from frequent changes.
With rapid satellite motions, the terrestrial users served by one satellite have to frequently switch to new satellites (thus new network interfaces and address) to retain its Internet access. %(every 120--125s per user, and 1000--6000 IP address changes per second in Starlink). 
As shown in Figure~\ref{fig:ip_change}, each user should change its logical IP address every 120--125s, and every 1000--6000 users per second should change their IP addresses as their serving satellites moves. 
%
\lixin{Update the number. Elaborate on the experiment methodology.}
Such frequent address changes will repetitively disrupt the TCP connections and upper-layer applications, thus negatively impacting the user experiences of satellite network services. 
\fi


\iffalse
\paragraphb{Unscalable and unstable network routing:} Traditional link-state routing suffers from (1) frequently re-convergence (Iridium) due to link switch; or (2) unacceptable converge to large-scale mega-constellation as new satellites are launched (Starlink, Kuiper). Both will lower the network usability.

\begin{compactitem}
\item A common solution to scale link-state routing is to divide the mega-constellation into ASes. However, this unavoidably incurs tradeoff between scalability and routing efficiency (detouring). 
\end{compactitem}
\fi

%\paragraphb{Frequent network topology change:} which causes traditional link-state routing to frequently re-convergence, and therefore low network service availability. 
%\lixin{Check in our empirical studies of OSPF here}

\iffalse
\begin{figure}[t]
\includegraphics[width=\columnwidth]{figures/unstable-mapping.pdf}
\caption{Unstable many-to-many mapping between terrestrial users and satellites.
\yuanjie{To be refined...}
}
\label{fig:unstable-mapping}
\end{figure}
\fi

\iffalse
\paragraphb{Unstable satellite-user mapping:}
The earth's rotation and its relative motion to satellites complicate the network routing. 
As exemplified in Figure~\ref{XXX}\guojie{Use a satellite sub-point trajectory of Starlink to showcase the many-to-many mapping.}, the satellite-user mapping is many-to-many, time-varying and highly dynamic: Each moving satellite serves more than one terrestrial user, while each user has choices of multiple access satellites each time. 
It is a challenging task to properly locate the satellite and terrestrial users for correct and efficient routing.
\fi

\paragraphb{How mega-constellation amplifies instability:}
Both stability issues will be worsen with more satellites.
For the terrestrial users, more satellites result in more frequent handoffs between satellites, thus causing more frequent IP address changes.
For the network, Figure~\ref{fig:usability} shows more satellites prolong the routing re-convergence on link change, thus decreasing the network usability. 
Moreover, more satellites complicate the dynamic routing between the moving satellites and terrestrial users (due to earth's rotation). 
Solutions for small LEO networks decades ago (\eg, virtual topology \cite{werner1997dynamic, chang1998fsa} and virtual nodes \cite{ekici2000datagram, ekici2001distributed}) cannot scale to the mega-constellations today due to their high complexity of computation, storage, or out-of-band control via specialized protocols. 

%First, as shown in Figure~\ref{fig:usability}, more satellites in mega-constellation prolong the routing re-convergence on link change, thus decreasing the network usability. 
%Second, more satellites result in more frequent changes of serving satellite by users, thus causing more frequent IP address changes.
%Last but not least, more satellites amplify the dynamic many-to-many mapping between the satellites and terrestrial users, thus further complicating the routing. 
\yuanjie{To be polished.}

\iffalse
\paragraphb{How {\em mega} constellation worsens above issues:} Many-to-many mappings between satellites and terrestrial users. 
\yuanjie{Criticize Starlink has more satellites than necessary (longer re-convergence time, more frequent IP changes, launch cost, space rubbish, visibility). Implicitly motivate \name to have less satellites}
\fi

==> challenge.tex <==
%\subsection{Deficiencies of Mega-Constellations Today}
\subsection{Unstable Mega-Constellations Today}
\label{sec:challenge}

The LEO mega-constellations today are primarily designed for enabling {\em full coverage} with low latency for the terrestrial users.
\del{Unfortunately, they fall short in enabling stable and efficient {\em inter-networking, addressing and routing}.}
\add{Since they are still at the early stages of deployment, they have not yet fully explored stable and efficient {\em inter-networking, addressing and routing}.}
With the high mobility of satellites and earth, networking with the existing mega-constellations suffers from three deficiencies of stability on the network and user sides:


\paragraphb{Unstable satellite network topology:}
Compared to the MEO/GEO satellites, LEO satellites at much lower altitude (typically $\leq$2,000 km) exhibit high mobility\footnote{According to Kepler's third law, for all satellites of the earth, the ratio between their orbital altitude and period $(R_E+H_s)^3/T_s^2$ is a constant.} and relative motions.
This results in frequent satellite network topology and inter-satellite link (ISL) changes.
It not only complicates the network routing in space, but also triggers repetitive re-convergence in link-state routing protocols and therefore significantly lowers the network usability.
%($\leq$10\% network availability for Starlink and Kuiper)\lixin{update the number}. 
Figure~\ref{fig:usability} illustrates the usability of mega-constellations using \textsf{motif}~\cite{bhattacherjee2019network}, a recently proposed LEO satellite inter-networking scheme.
\lixin{Methodology of the experiments}
It shows that, all mega-constellations today suffer from $\leq10\%$ network availability\footnote{A common solution to scale link-state routing is to divide the mega-constellation into ASes. However, this unavoidably incurs tradeoff between scalability and routing efficiency (detouring). \yuanjie{To be polished.}}.\lixin{update the number}

\lixin{For Iridium, show the empirical results of low network usable time. For Starlink, Kuiper and Telesat, show the convergence time \wrt number of satellites using \textsf{motif}.}

\begin{figure}[t]
\subfloat[Starlink]{
\includegraphics[width=0.5\columnwidth]{figures/usibility.eps}
}
\subfloat[Kuiper]{
\includegraphics[width=0.5\columnwidth]{figures/kuiper.eps}
\label{fig:base-case}
}
\caption{Low network usability in state-of-the-art constellations.} %\lixin{(1) Why low availability (<80\%) when there are very few satellites? (2) Why very slow usability decrement as the constellation becomes larger? (3) How about motif in CoNEXT'19?}
\label{fig:usability}
\end{figure}

\paragraphb{Unstable user addressing:} 
The classical logical network addressing suffers from frequent changes.
With rapid satellite motions, the terrestrial users served by one satellite have to frequently switch to new satellites (thus new network interfaces and address) to retain its Internet access. %(every 120--125s per user, and 1000--6000 IP address changes per second in Starlink). 
As shown in Figure~\ref{fig:ip_change}, each user should change its logical IP address every 120--125s, and every 1000--6000 users per second should change their IP addresses as their serving satellites moves. 
%
\lixin{Update the number. Elaborate on the experiment methodology.}
Such frequent address changes will repetitively disrupt the TCP connections and upper-layer applications, thus negatively impacting the user experiences of satellite network services. 


\begin{figure}[t]
\includegraphics[width=\columnwidth]{figures/ip_change.eps}
\caption{Frequent changes of terrestrial users' IP addresses in state-of-the-art LEO mega-constellations. \lixin{Is IP change \wrt altitude a key point of this paper?}}
\label{fig:ip_change}
\end{figure}



\iffalse
\paragraphb{Unscalable and unstable network routing:} Traditional link-state routing suffers from (1) frequently re-convergence (Iridium) due to link switch; or (2) unacceptable converge to large-scale mega-constellation as new satellites are launched (Starlink, Kuiper). Both will lower the network usability.

\begin{compactitem}
\item A common solution to scale link-state routing is to divide the mega-constellation into ASes. However, this unavoidably incurs tradeoff between scalability and routing efficiency (detouring). 
\end{compactitem}
\fi

%\paragraphb{Frequent network topology change:} which causes traditional link-state routing to frequently re-convergence, and therefore low network service availability. 
%\lixin{Check in our empirical studies of OSPF here}

\begin{figure}[t]
\includegraphics[width=\columnwidth]{figures/unstable-mapping.pdf}
\caption{Unstable many-to-many mapping between terrestrial users and satellites.
\yuanjie{To be refined...}
}
\label{fig:unstable-mapping}
\end{figure}

\paragraphb{Unstable satellite-user mapping:}
The earth's rotation and its relative motion to satellites complicate the network routing. 
As exemplified in Figure~\ref{XXX}\guojie{Use a satellite sub-point trajectory of Starlink to showcase the many-to-many mapping.}, the satellite-user mapping is many-to-many, time-varying and highly dynamic: Each moving satellite serves more than one terrestrial user, while each user has choices of multiple access satellites each time. 
It is a challenging task to properly locate the satellite and terrestrial users for correct and efficient routing.


\paragraphb{How instability is amplified in {\em mega}-constellation:}
All the above stability issues are amplified with more satellites in the mega-constellation.
First, as shown in Figure~\ref{fig:usability}, more satellites in mega-constellation prolong the routing re-convergence on link change, thus decreasing the network usability. 
Second, more satellites result in more frequent changes of serving satellite by users, thus causing more frequent IP address changes.
Last but not least, more satellites amplify the dynamic many-to-many mapping between the satellites and terrestrial users, thus further complicating the routing. 
\yuanjie{To be polished.}

\iffalse
\paragraphb{How {\em mega} constellation worsens above issues:} Many-to-many mappings between satellites and terrestrial users. 
\yuanjie{Criticize Starlink has more satellites than necessary (longer re-convergence time, more frequent IP changes, launch cost, space rubbish, visibility). Implicitly motivate \name to have less satellites}
\fi

==> concl-v1.tex <==
\section{Conclusion}
\label{sect:concl}



This paper presents \name, a new LEO mega-constellation for networking in space. 
%To combat the unstable addressing and routing due to high mobility of massive satellites and earth, 
%\name explores a paradigm shift from the {\em coverage-first} to {\em networking-first} mega-constellation design. 
\name aims for stable and scalable network topology, addressing, and routing in the presence of high satellite mobility and earth's rotation.
It offers a time-invariant recursive interconnection structure over the Rosette constellation with earth-repeat orbits, and devises hierarchical geographical cells to stabilize the network addressing. 
\name supports efficient single-path routing with bounded latency, multi-path routing for high performance and fault tolerance, and on-demand incremental expansion with fewer satellites.

\name represents a paradigm shift from the {\em coverage-first} to {\em networking-first} mega-constellation design. 
Compared to terrestrial networks, the satellite networks are much harder to modify after the satellites are launched to space. 
%\name is an initial effort for revisiting the fundamental satellite network design.
As we are still at the early stages of networking in space, it is necessary to systematically explore the issues and spaces for the mega-constellation design, and ensure that the constellation is well suited for inter-networking in space. 
We hope \name could call for the community's attention, and stimulate more research efforts for stable and efficient networking in space at scale. 

%We are still at the early stages of the Internet in space. 
%As more and more LEO mega-constellations are underway, it is the time for us to rethink 




\iffalse
\begin{compactitem}
\item A fundamental design paradigm transition: Constellation for {\em coverage} $\rightarrow$ constellation for {\em networking}. 

\item Stable constellation is made {\em possible} for LEO satellites.
\end{compactitem}


{Highlight the following in the paper
\begin{compactitem}
\item Scalable low earth orbit ({\bf LEO}) constellation for high performance;
	\begin{compactitem}
	\item LEO was considered harder to use than MEO/GEO due to high mobility;
	\end{compactitem}
\item \#1 goal is {\bf network routing, not coverage} (although full coverage is also guaranteed);
	\begin{compactitem}
	\item This outperforms traditional Rosette/Walker constellation
	\item Networking for mega-constellation is still {\em at early stages}. This work is {\em not} intended to blame existing constellations. Instead, it seeks to provide a new perspective to help the community rethink the networking in space.
	\end{compactitem}	
\item On-demand mega constellation; 
	\begin{compactitem}
	\item Less satellites than Starlink, but still high networking performance;
	\end{compactitem}

\item Robust to {\bf high mobility} in satellite and earth; 
	\begin{compactitem}
	\item LEO was considered harder to use than MEO/GEO due to high mobility;
	\end{compactitem}
%\item Networking in space, rather than coverage for traditional constellations; 
\item Addressing in space (based on Rosette and hypercube);
\item Multi-paths (fault tolerance and performance); 
	\begin{compactitem}
	\item {\bf Mobility} increases fault tolerance in presence of satellite or link failures;
	\end{compactitem}
\end{compactitem}}
\fi

==> construction-v2.tex <==
\subsection{\name Construction}
\label{sec:construction}

\begin{figure*}[t]
\vspace{-10mm}
\centering
%\subfloat[\textsf{Shift(\name, t)} in Algorithm~\ref{algo:construction}]{%\wei{Replace $Q$ with $2^k$. Be consistent with Algorithm 1}]{
\subfloat[\textsf{Shift(\name, t)} in construction]{
\includegraphics[width=.3\textwidth]{figures/rotate.pdf}
}
\subfloat[Logical network topology of $\name_k$]{
%\includegraphics[width=.6\textwidth]{figures/recursion-v1.pdf}
\includegraphics[width=.6\textwidth]{figures/recursion-v2.pdf}
}
\vspace{-3mm}
\subfloat[Physical constellation in 3D space]{
\includegraphics[width=.3\textwidth]{figures/3D-view.pdf}
}
\subfloat[Hierarchical geographical cells by sub-points of satellites with ground-track repeat orbits.]{ %\wei{Replace it with high-resolution figure}]{
\includegraphics[width=.6\textwidth]{figures/subsate-trajectory.pdf}
\label{fig:construction:cell}
}


\caption{Recursive construction of \name.}
\label{fig:construction}
\end{figure*}

\begin{algorithm}[t]
   \centering
        \begin{algorithmic}[1]% The number tells where the line numbering should start
    	\Require{A Rosette constellation $(N,N,m)$, and a \name level $k\geq0$}
	\Ensure{$\name_k$}
	\State $\name_0=(N,N,m)$ Rosette constellation;
	\For{j=1 to k}
	\State $\name_j=\{\}$; 
	\For{i= 0 to N-1}  \textcolor{gray}{\Comment{{\em\tiny Step 1: Construct $N$ $\name_{j-1}$s}}}
	\State $\name_{j-1}^i=\textsf{Shift}(\name_{j-1}, \frac{2\pi}{N^j})$;
	\State $\name_j$.append($\name_{j-1}^i$);
	\EndFor
	\For{i=0 to N-1}  \textcolor{gray}{\Comment{{\em\tiny Step 2: Inter-connect $\name_{j-1}$s}}}
	\For{each satellite $S_{i}$ in $\name_{j-1}^i$}
	\State Connect $S_i$ to $S_{(i+1\mod N)}$ in $\name_{j-1}^{(i+1\mod N)}$;
	\EndFor
	\EndFor
	\EndFor
	
	\State \Return $\name_k$;
	
	
    \end{algorithmic}
    \caption{\name construction. %\todo{Everyone: Please check the correctness.}
    }
    \label{algo:construction}
\end{algorithm}

\name adopts the Rosette constellation as a base case, but extends it recursively with inter-satellite links. 
A $\name_0$ is a classic $(N,N,m)$ Rosette constellation in $\S$\ref{sec:rosette-primer}, with inter-satellite links in adjacent satellites (exemplified in Figure~\ref{fig:base-case}) and ground-track repeat orbits for all satellites (\ie, $T_s=T_E/(N-m)$).
%\wei{How to choose the baseline?}
A $\name_k$ ($k\geq1$) constellation is constructed recursively from $N$ $\name_{k-1}$ constellations.
Algorithm~\ref{algo:construction} shows \name construction.
It takes two phases (exemplified in Figure~\ref{fig:construction}):
\yuanjie{The \name construction in Algorithm~\ref{algo:construction} does not mandate the base case in Figure~\ref{fig:base-case}, which only uses local links and results in detouring when inter-orbit links cannot be established (Theorem~\ref{thm:hop}). By extending the base case to non-local links, \name can achieve similar lower latency to motif.}

\paragraphe{(1) Construct $N$ $\name_{k-1}$s:} 
The $\name_{k-1}$ constellations are numbered from 0 to $N-1$, denoted as $\name_{k-1}^0$, $\name_{k-1}^1$, $...$, $\name_{k-1}^{N-1}$. 
A $\name_{k-1}^i$ is obtained by first duplicating a $\name_{k-1}^0$, and then shifting $\name_{k-1}$ by a time interval $t_k=\frac{T_S}{N^k}$. This is equivalent to shifting each satellite in $\name_{k-1}^0$ by a phase $x_k=\frac{2\pi}{T_s}\cdot t_k=\frac{2\pi}{N^k}$. %\todo{Check this shift}.
In this way, it is easy to see that each satellite $S_j$ in $\name_{k-1}^0$ is replicated $N$ times on the same orbit. denoted as $S_j^0,S_j^1,...S_j^{N-1}$.

\paragraphe{(2) Interconnect $\name_{k-1}$s:} We next bridge $\name_{k-1}$s with {\em intra-orbit} inter-satellite links only.
For each satellite $S_i$ in $\name_{k-1}^i$ ($i=0,1,...,N-1$), we add a link to $S_{(i+1\mod N)}$ (in the same orbit as $S_{i}$) in $\name_{k-1}^{(i+1\mod N)}$. 
This creates a circle among satellites on the same orbit.

%It is also easy to verify that, every $\name_k$ is also a Rosette constellation in $\S$\ref{sec:rosette-primer}. % with parameter $(N^{k+1},N, \frac{m}{N^k})$.

%\yuanjie{Finalize the base case ($\name_0$): A circle, a hypercube, or arbitrary Rosette constellation? The \underline{prioritized} goals are (1) guarantee always-on stable ISLs; then (2) mitigate the detouring whenever possible.}

%It is easy to see that each $\name_k$ has $N^{k+1}$ satellites. 


%A $\name_{k-1}^i$ is obtained by first replicating $\name_{k-1}^0$, and then shifting $\name_{k-1}^0$ by a time shift $t_k=\frac{T_S}{N^k}$ or equivalent phase $x_k=\frac{2\pi}{T_s}\cdot t_k=\frac{2\pi}{N^k}$\todo{Check this shift}.


%\fixme{Why hypercube? Why inter-networking this way? Is it the {\em only} stable inter-networking?}

%\lixin{Baseline construction, which guarantees (1) always-on and stable ISL; and (2) minimizes the altitude.}


%\yuanjie{Elaborate on design procedure of \name: Given latency (altitude) demand and hardware constraint for elevation angle, derive the minimal satellites needed for full coverage, then find the closest \name to construct.}

%\wei{The formula to decide the number of satellites given altitude (latency) and elevation angle.}

%\todo{Compare \name with state-of-the-arts (Starlink, Kuiper, OneWeb, \etc) \wrt no. satellites, stability, scalability, routing, \etc. A table would be helpful.}

==> construction.tex <==
\subsection{\name Construction}
\label{sec:construction}

\begin{figure*}[t]
\centering
\subfloat[\textsf{Shift(\name, t)} in Algorithm~\ref{algo:construction}]{%\wei{Replace $Q$ with $2^k$. Be consistent with Algorithm 1}]{
\includegraphics[width=.3\textwidth]{figures/rotate.pdf}
}
\subfloat[Logical network topology of $\name_k$]{
\includegraphics[width=.6\textwidth]{figures/recursion-v1.pdf}
}
\vspace{-3mm}
\subfloat[Physical constellation in 3D space]{
\includegraphics[width=.3\textwidth]{figures/3D-view.pdf}
}
\subfloat[Hierarchical geographical cells by sub-points of satellites with earth-repeat orbits.]{ %\wei{Replace it with high-resolution figure}]{
\includegraphics[width=.6\textwidth]{figures/subsate-trajectory.pdf}
\label{fig:construction:cell}
}


\caption{Recursive construction of \name.}
\label{fig:construction}
\end{figure*}

\begin{algorithm}[t]
   \centering
        \begin{algorithmic}[1]% The number tells where the line numbering should start
    	\Require{A Rosette constellation $(N,N,m)$, and a \name level $k\geq0$}
	\Ensure{$\name_k$}
	\State $\name_0=(N,N,m)$ Rosette constellation;
	\For{j=1 to k}
	\State $\name_j=\{\}$; 
	\For{i= 0 to N-1}  \textcolor{gray}{\Comment{{\em\tiny Step 1: Construct $N$ $\name_{j-1}$s}}}
	\State $\name_{j-1}^i=\textsf{Shift}(\name_{j-1}, \frac{2\pi}{N^j})$;
	\State $\name_j$.append($\name_{j-1}^i$);
	\EndFor
	\For{i=0 to N-1}  \textcolor{gray}{\Comment{{\em\tiny Step 2: Inter-connect $\name_{j-1}$s}}}
	\For{each satellite $S_{i}$ in $\name_{j-1}^i$}
	\State Connect $S_i$ to $S_{(i+1\mod N)}$ in $\name_{j-1}^{(i+1\mod N)}$;
	\EndFor
	\EndFor
	\EndFor
	
	\State \Return $\name_k$;
	
	
    \end{algorithmic}
    \caption{\name construction. %\todo{Everyone: Please check the correctness.}
    }
    \label{algo:construction}
\end{algorithm}

\name adopts the Rosette constellation as a base case, but is defined recursively. 
A $\name_0$ is a classic $(N,N,m)$ Rosette constellation in $\S$\ref{sec:rosette-primer}, with inter-satellite links in adjacent satellites (exemplified in Figure~\ref{fig:base-case}) and earth-repeat orbits for all satellites (\ie, $T_s=T_E/(N-m)$).
%\wei{How to choose the baseline?}
A $\name_k$ ($k\geq1$) constellation is constructed recursively from $N$ $\name_{k-1}$ constellations.
Algorithm~\ref{algo:construction} shows \name construction.
It takes two phases (exemplified in Figure~\ref{fig:construction}):
\yuanjie{The \name construction in Algorithm~\ref{algo:construction} does not mandate the base case in Figure~\ref{fig:base-case}, which only uses local links and results in detouring when inter-orbit links cannot be established (Theorem~\ref{thm:hop}). By extending the base case to non-local links, \name can achieve similar lower latency to motif.}

\paragraphe{(1) Construct $N$ $\name_{k-1}$s:} 
The $\name_{k-1}$ constellations are numbered from 0 to $N-1$, denoted as $\name_{k-1}^0$, $\name_{k-1}^1$, $...$, $\name_{k-1}^{N-1}$. 
A $\name_{k-1}^i$ is obtained by first duplicating a $\name_{k-1}^0$, and then shifting $\name_{k-1}$ by a time interval $t_k=\frac{T_S}{N^k}$. This is equivalent to shifting each satellite in $\name_{k-1}^0$ by a phase $x_k=\frac{2\pi}{T_s}\cdot t_k=\frac{2\pi}{N^k}$. %\todo{Check this shift}.
In this way, it is easy to see that each satellite $S_j$ in $\name_{k-1}^0$ is replicated $N$ times on the same orbit. denoted as $S_j^0,S_j^1,...S_j^{N-1}$.

\paragraphe{(2) Interconnect $\name_{k-1}$s:} We next bridge these $N$ $\name_{k-1}$s with {\em intra-orbit} inter-satellite links only.
For each satellite $S_i$ in $\name_{k-1}^i$ ($i=0,1,...,N-1$), we add a link to $S_{(i+1\mod N)}$ (in the same orbit as $S_{i}$) in $\name_{k-1}^{(i+1\mod N)}$. 
This creates a circle among satellites on the same orbit.

It is straightforward to verify that a $\name_k$ has $N^{k+1}$ satellites and $(k+1)N^{k+1}$ inter-satellite links.
%It is also easy to verify that, every $\name_k$ is also a Rosette constellation in $\S$\ref{sec:rosette-primer}. % with parameter $(N^{k+1},N, \frac{m}{N^k})$.

%\yuanjie{Finalize the base case ($\name_0$): A circle, a hypercube, or arbitrary Rosette constellation? The \underline{prioritized} goals are (1) guarantee always-on stable ISLs; then (2) mitigate the detouring whenever possible.}

\paragraphb{Minimum altitude to deploy a $\name_k$:}
To ensure the full coverage and always-on inter-satellite links, the satellites in a $\name_k$ should be deployed at an appropriate altitude.
To derive the altitude, consider the inter-satellite link that is the most vulnerable to disconnection, which is between the satellites on different orbits near the equator.
To ensure this link is always on, the satellites' altitude should satisfy $(H+R_E)\cos(\frac{\alpha}{2})>(R_E+H_A)$, where $\alpha=\sqrt{(\frac{2\pi}{N})^2+(\frac{2\pi}{N^k})^2}$ is the angle $\angle S_1OS_2$, $O$ is the earth center, $R_E$ is earth radius and $H_A$ is height of the atmosphere . 
%where $R_E$ means radius of the earth and $H_A$ means height of the atmosphere.
Table~\ref{tab:altitude} exemplifies the minimum altitude of satellites for $\name_k$ when $N=8,m=6,\phi=25^\circ$.


\iffalse
Table~\ref{tab:altitude}.
\wei{To ensure full coverage and always-on ISL, show the formula of computing the minimum altitude of the constellation. Exemplify the height with 8, 64, 512, and 4096 satellites in a table. Draft:To ensure full coverage, $\sec R_{min}=\sqrt{3}\tan{\left(\frac{\pi}{6}\frac{N_{min}}{N_{min}-2}\right)}$ and  $\tan\phi=\frac{\cos R_{min}-R_E/(R_E+H)}{\sin R_{min}}$. Same as On-demand \name size selection.
To ensure the ISLs can be established at all times, we consider the ISL established between satellites  near the equator, which belong to different orbits, because the ISL is the longest at this time. At this time, connect the center of the earth to the two satellites, and the angle $\alpha=\sqrt{(\frac{2\pi}{N})^2+(\frac{2\pi}{N^k})^2}$. To ensure the ISL can be established at this time, it needs to meet $(H+R_E)\cos(\frac{\alpha}{2})>(R_E+H_A)$, where $R_E$ means radius of the earth and $H_A$ means height of the atmosphere.}  
\fi

\begin{table}[t]
\caption{\name's satellites' altitude when $N$=8, $m$=6, and the elevation angle $\phi=25^{\circ}$.}%\lixin{Check if these numbers are correct.}
\label{tab:altitude}
\resizebox{1\columnwidth}{!}{{
\begin{tabular}{|c|c|c|c|c|}
\hline
& {\bf Number of} & {\bf Min. altitude for} & {\bf Ground-to-} & {\bf Average cell}\\
& {\bf satellites} & {\bf full coverage (km)} & {\bf satellite RTT (ms)} & {\bf size (km$^2$)}\\
\hline
{\bf $\name_0$} & 8 & 11848.46 & 78.99 & \\
\hline
	{\bf $\name_1$} & 64 & 1259.52 & 8.40 & \\
\hline	
{\bf $\name_2$} & 512 &  335.33 & 2.24 & \\
\hline
{\bf $\name_3$} & 4096 & 107.63 & 0.72 & \\
\hline
\end{tabular}
}}
%\caption{Three main test phone models (Android). }
\end{table}




%\paragraphb{Altitudes and numbers of satellites needed:}
\paragraphb{On-demand \name size selection:}
A satellite operator can select the proper \name size that can ensure full coverage {\em and} meet its network latency demands.
Algorithm~\ref{algo:layout} illustrates the size selection based on the ground-to-space round trip latency demand \textsf{RTT}, and the minimum elevation angle $\phi$ (constrained by the satellite and device hardware's capability).
The operator can first specify the desired altitude of the satellites $H=c\cdot\textsf{RTT}/2$, where $c$ is the light speed through the atmosphere. 
With the minimum elevation angle $\phi$, one we derive the minimal per-satellite coverage $R_{min}$ in the unit of great circle range:
$\tan\phi=\frac{\cos R_{min}-R_E/(R_E+H)}{\sin R_{min}}$.
With $R_{min}$ the operator can derive the minimal number of satellites needed for a Rosette constellation to guarantee full coverage:
$\sec R_{min}=\sqrt{3}\tan{\left(\frac{\pi}{6}\frac{N_{min}}{N_{min}-2}\right)}$.
Then given the $\name_0$ parameter $N$, the operator can choose the level of \name as $k=\lceil{\log_N{N_{min}}}\rceil-1$.
%\wei{Check if anything is missing.}

%\paragraphb{How many layers do we need?}

\iffalse
\paragraphb{Two physical realizations of \name:}
\todo{Move this part to $\S$\ref{sec:deployment}.}

\begin{compactitem}
\item {\bf Layered realization:} $\name_{k-1}$ as MEO (Backbone), and $\name_k$ as LEO (access network). The backbone $\name_{k-1}$ at higher altitude connects all $\name_k$ at lower altitude. This facilitates incremental expansion, and mitigates the detouring in $\name_k$ (to be detailed in $\S$\ref{sec:routing-sat}).

\item {\bf Flat realization:} All satellites reside at the same altitudes. This approaches do not need high-altitude satellites, thus shorter ground-to-satellite RTT. But it is not friendly to incremental expansion\yuanjie{Really?}: All satellites should be available before enabling $\name_k$. Besides, detouring can happen (see Theorem~\ref{thm:hop}--\ref{thm:latency}).
\end{compactitem}
\fi


\begin{algorithm}[t]
   \centering
        \begin{algorithmic}[1]% The number tells where the line numbering should start
    	\Require{Ground-to-satellite round-trip demand \textsf{RTT}, minimum available elevation angle $\phi$, and Rosette constellation parameter $N$}
	\Ensure{The minimum number of layers $k$ and satellites $N_k$  for \name to guarantee full coverage}
	\State Compute satellite altitude $H=c\cdot\textsf{RTT}/2$; \todo{Replace $c$}
	\State Find each satellite's minimum coverage $R_{min}$ in the unit of great circle range: 
	$$\tan\phi=\frac{\cos R_{min}-R_E/(R_E+H)}{\sin R_{min}}$$
	
	\State Decide the minimum number of satellites to guarantee full coverage:
	
	$$\sec R_{min}=\sqrt{3}\tan{\left(\frac{\pi}{6}\frac{N_{min}}{N_{min}-2}\right)}$$
	
	\State Decide the minimum number of layers $k$ for \name:
	
	 $$k=\lceil{\log_N{N_{min}}}\rceil-1$$
	 
	
	\State Decide the minimum number of satellites in \name: $N_k=N^{k+1}$;
	 
	
	
    \end{algorithmic}
    \caption{On-demand \name size selection. \todo{Everyone: Please check the correctness.}}
    \label{algo:layout}
\end{algorithm}

%It is easy to see that each $\name_k$ has $N^{k+1}$ satellites. 


%A $\name_{k-1}^i$ is obtained by first replicating $\name_{k-1}^0$, and then shifting $\name_{k-1}^0$ by a time shift $t_k=\frac{T_S}{N^k}$ or equivalent phase $x_k=\frac{2\pi}{T_s}\cdot t_k=\frac{2\pi}{N^k}$\todo{Check this shift}.


%\fixme{Why hypercube? Why inter-networking this way? Is it the {\em only} stable inter-networking?}

%\lixin{Baseline construction, which guarantees (1) always-on and stable ISL; and (2) minimizes the altitude.}


%\yuanjie{Elaborate on design procedure of \name: Given latency (altitude) demand and hardware constraint for elevation angle, derive the minimal satellites needed for full coverage, then find the closest \name to construct.}

%\wei{The formula to decide the number of satellites given altitude (latency) and elevation angle.}

%\todo{Compare \name with state-of-the-arts (Starlink, Kuiper, OneWeb, \etc) \wrt no. satellites, stability, scalability, routing, \etc. A table would be helpful.}

==> discuss.tex <==
\section{Discussion}
\label{sect:discuss}

\p{Misc issues for \name, such as incremental deployment, backward compatibility with classical IP address, the impact of imperfect prediction, orbits perturbation, polar orbit, ISL links between orbits, ...}


\paragraphb{Multicast/broadcast addressing:} \name so far focuses on unicast addressing, XXX. \todo{Implications for multicast/broadcast on satellites?}

==> empirical-study.tex <==
\subsection{How Good is Existing IP Address?}
\label{problem:empirical}

%\paragraphb{How serious are these problems in reality?}

We conduct empirical validations over realistic mega constellations and state-of-the-art routing protocols
\todo{Use experiments to give people a {\bf first impression} of how bad the logical IP is for satellites.}

\paragraphe{$\bullet$ Impact on the users:}

\paragraphe{$\bullet$ Impact on the network:}

==> eval-micro-v2.tex <==
\subsection{System Overhead}
\label{sect:eval:micro}


\paragraphb{Packet processing latency:}

\paragraphb{CPU overhead:} Satellite is resource-constrained

\paragraphb{Storage overhead}

\begin{compactitem}
\item {\bf Routing table size:}
\item {\bf Cell ID table size:}
\end{compactitem}


\iffalse
\todo{Place holders only. To be discussed and refined.}

\paragraphb{Locality:}

\paragraphb{Stability:}

\paragraphb{Clustering:}
\fi



==> eval-micro.tex <==
\subsection{Efficiency and Overhead}
\label{sect:eval:micro}


\paragraphb{Packet processing latency:}

\paragraphb{CPU overhead:} Satellite is resource-constrained


\iffalse
\todo{Place holders only. To be discussed and refined.}

\paragraphb{Locality:}

\paragraphb{Stability:}

\paragraphb{Clustering:}
\fi



==> eval-overall-v2.tex <==
%\subsection{Routing Performance}
\subsection{Routing in \name}
\label{sect:eval:overall}


%\subsubsection{Routing in space}


\paragraphb{Single-path routing:}

\begin{compactenum}

\item {\bf Hop and delay:} Figure~\ref{fig:delay_hop_diff}
%\lixin{Since ISL length varies over time, the routing latency should also vary periodically. Show this trend.}

\item {\bf Routing stretch:} How close is \name routing to the optimal shortest path routing?


\end{compactenum}


\paragraphb{Multi-path routing:} Figure~\ref{fig:multi_delay_cdf}. \todo{de-emphasize it.}

\begin{compactenum}
\item {\bf Variance of latency among paths:}
\item {\bf Graceful degradation \wrt faults:}
\end{compactenum}

\begin{figure}[t]
\subfloat[Experimental Results]{
\includegraphics[width=0.53\columnwidth]{figures/225delay_hop.eps}
\label{fig:delay_hop}
}
\subfloat[CDF]{
\includegraphics[width=0.47\columnwidth]{figures/225delay_cdf.eps}
\label{fig:delay_cdf}
}
\caption{\name's near-optimal shorting.}
\label{fig:delay_hop_diff}
\end{figure}

\begin{figure}[t]
\includegraphics[width=.8\columnwidth]{figures/225delay_multi.eps}
\caption{\name's multi-path routing.}
\label{fig:multi_delay_cdf}
\end{figure}


%\subsubsection{Routing for terrestrial users}


\iffalse
\todo{Place holders only. To be discussed and refined.}

\paragraphb{IP changes \wrt mobility:}

\paragraphb{Network availability:}

\paragraphb{Capacity:}

\paragraphb{Latency:}
\fi



==> eval-overall-v3.tex <==
%\subsection{Routing Performance}
\subsection{Networking in \name}
\label{sect:eval:overall}

We next evaluate the networking in \name. 
It has been proved in $\S$\ref{sec:address}--$\S$\ref{sec:routing} that \name does not suffer from frequent user IP address changes or routing re-convergence (thus low network usability) in $\S$\ref{sec:challenge}.
So this section focuses on the efficiency of addressing and routing instead.
%So we quantify the efficiency of addressing and routing instead.




\paragraphb{Addressing:} No frequent IP changes in $\S$\ref{sec:challenge}


\paragraphe{$\circ$ Stability:} 

\begin{compactitem}
\item {\em Satellite address:} Time-invariant.
\item {\em Ground address:} Stable unless the terrestrial user moves to a new area (rare according to Table~\ref{tab:altitude}).
\end{compactitem}


\paragraphe{$\circ$ Efficiency:} 

\begin{compactitem}
\item {\em CPU:}
\item {\em Storage:}
\end{compactitem}


\paragraphb{Routing:} No re-convergence and low usability in $\S$\ref{sec:challenge}

\paragraphe{$\circ$ Stability:}

%\subsubsection{Routing in space}

\paragraphe{$\circ$ Efficiency:}

\begin{compactitem}


\item {\em Routing stretch:} Figure~\ref{fig:delay_hop_diff}. How close (hop and delay) is \name routing to the shortest path routing?

\item {\em Multi-path routing:} Figure~\ref{fig:multi_delay_cdf}. \todo{de-emphasize it.}


\end{compactitem}

\iffalse
\begin{compactenum}
\item {\bf Variance of latency among paths:}
\item {\bf Graceful degradation \wrt faults:}
\end{compactenum}
\fi

\begin{figure}[t]
\subfloat[Experimental Results]{
\includegraphics[width=0.53\columnwidth]{figures/225delay_hop.eps}
\label{fig:delay_hop}
}
\subfloat[CDF]{
\includegraphics[width=0.47\columnwidth]{figures/225delay_cdf.eps}
\label{fig:delay_cdf}
}
%\caption{\name's near-optimal shorting.}
\caption{\name's routing performance.}
\label{fig:delay_hop_diff}
\end{figure}

\begin{figure}[t]
\includegraphics[width=.8\columnwidth]{figures/225delay_multi.eps}
\caption{\name's multi-path routing.}
\label{fig:multi_delay_cdf}
\end{figure}


\begin{figure}[t]
\subfloat[Process Latency for per Packet]{
\includegraphics[width=0.5\columnwidth]{figures/process_latency.eps}
\label{fig:process_latency}
}
\subfloat[Bandwidth]{
\includegraphics[width=0.5\columnwidth]{figures/iperf.eps}
\label{fig:iperf}
}
%\caption{\name's near-optimal shorting.}
\caption{\name's routing performance.}
\label{fig:performance}
\end{figure}
    

==> eval-overall.tex <==
\subsection{Overall Merits}
\label{sect:eval:overall}

\paragraphb{Number of satellites:} Less satellites than Starlink, Kuiper, \etc to enable full coverage under the same parameter settings

\paragraphb{Stability:} Less (or no) changes of ISLs in high satellite and earth mobility

\subsubsection{Routing in space}


%\paragraphb{Addressing size:}

\paragraphb{Single-path routing:}

\begin{compactenum}
\item {\bf Hops:} \wei{Proved by theorem?}
\item {\bf Propogation delay:} 
%\lixin{Since ISL length varies over time, the routing latency should also vary periodically. Show this trend.}


\item {\bf Routing stretch:} How close is \name routing to the optimal shortest path routing?
\end{compactenum}


\paragraphb{Multi-path routing:}

\begin{compactenum}
\item {\bf }
\item {\bf Graceful degradation \wrt faults:}
\end{compactenum}


\iffalse
\paragraphb{Locality:} How close is \name routing to the optimal shortest path routing?

\paragraphb{Clustering:}

\paragraphb{Multi-path routing:} Throughput boosting with multi-path routing

\paragraphb{Fault-tolerant routing:} Average throughput with random ISL/satellite failures
\fi

\subsubsection{Routing for terrestrial users}


\iffalse
\todo{Place holders only. To be discussed and refined.}

\paragraphb{IP changes \wrt mobility:}

\paragraphb{Network availability:}

\paragraphb{Capacity:}

\paragraphb{Latency:}
\fi



==> eval-v2.tex <==
\section{Evaluation}
\label{sect:eval}

%We assess \name's overall merits for users and network ($\S$\ref{sect:eval:overall}),
%and validate its properties for its key components ($\S$\ref{sect:eval:micro}).

%We characterize \name's key properties ($\S$\ref{sec:eval:characteristics}), evaluate its routing performance ($\S$\ref{sect:eval:overall}) and system overhead ($\S$\ref{sect:eval:micro}).
We evaluate the efficiency and overhead of \name's network structure ($\S$\ref{sec:eval:characteristics}), addressing ($\S$\ref{sec:eval:addr}) and routing  ($\S$\ref{sec:eval:routing}). 

\begin{figure}[t]
\vspace{-5mm}
\includegraphics[width=.7\columnwidth]{figures/prototype-v2.pdf}
\vspace{-2mm}
\caption{Hardware-in-the-loop experimental setup.}
\label{fig:setup}
\end{figure}

\paragraphb{Prototype:}
We prototype an IPv6-based addressing and routing suite for \name using Quagga~\cite{quagga}.
\add{Specifically, by extending the Quagga 0.99.23 version and modifying the packet processing module of Linux kernel 3.10.0 version, we deployed the \name prototype on 6 Dell EMC PowerEdge R740 servers.
These prototype implementation takes about 13K lines of C. }
Figure~\ref{fig:setup} illustrates our implementation.
At the control plane, we realize \name's hierarchical satellite/user address schemes, and embed them into the standard IPv6 address as shown in Figure~\ref{fig:user-address}.
We also implement Algorithm~\ref{algo:single-path-routing} to compute the next hop and routing table entry for a given destination. 
At the data plane, we reuse the standard IPv6 routing table and forwarding engine for prefix-based \name routing in $\S$\ref{sec:routing-sat}.
At runtime, an IPv6 packet with \name address will be forwarded to the user plane.
If the routing table does not have a next-hop entry for this address, it will be relayed to the control plane.
The control plane will parse the IPv6 address to get the \name address, run Algorithm~\ref{algo:single-path-routing} for this address, generate and install the routing table entry, and then forward the packet.
For later packets with the same \name address, they will be directly forwarded by routing table lookup at the data plane.
%\lixin{Please elaborate on the Quagga version, Linux version, and implementation details (\eg, lines of code), number of servers/mininets, \etc.}
\yuanjie{How ``close'' is this emulation to the real satellites?}
%Besides IPv6, \name's geographical user address can also be embedded into other future Internet designs such as SRv6, NDN~\cite{zhang2014named,jacobson2009networking}, MobilityFirst \cite{mobilityfirst}, SCION \cite{zhang2011scion}, and XIA \cite{han2012xia}.



\paragraphb{Experimental setup:}
Given our limited capability of launching massive satellites to space, we conduct a hardware-in-the-loop, trace-driven emulation for \name. 
We use \textsf{StarPerf} \cite{lai2020starperf} to emulate the mega-constellation with \name setup and real TLE orbit information of Starlink, Kuiper, TeleSat, and Iridium from Space-Track \cite{space-track}.
The emulator will generate the runtime satellite motions, earth rotations, inter-satellite link qualities (delay, loss, and throughput) based on the well-established celestial mechanics.
We use a \add{6}-server testbed with \textsf{Mininet} \cite{mininet} to create virtual satellites with \name protocol suite that operate under the emulated satellite trajectory.
We characterize \name's key properties with emulated traces, compare them with state-of-the-art mega-constellations, evaluate the routing performance and quantify the system overhead with our Quagga-based protocol suite.
\lixin{More details needed: server model and quantity; statistics of state-of-the-art mega-constellations; testbed topology (with a photo?)}


%\todo{Evaluation metrics, scenarios, baseline, and methodology. Would be nice if the evaluation can cover some use cases in $\S$\ref{sec:back:case}.}

\paragraphb{Ethics:} This work does not raise any ethical issues. %\yuanjie{mandatory according to SIGCOMM CFP}

\input{eval-characteristics}
%\input{eval-overall-v2} % 01/18/21: Re-position to routing only
%\input{eval-overall-v3} % 01/21/21: Re-organization, highlight stability, de-emphasize multi-path
%\input{eval-micro-v2} % 01/18/21: Re-position to system overhead only
\input{eval-addr}
\input{eval-routing}
%\input{eval-overall} % End-to-end evaluation from user/network's perspective
%\input{eval-micro}   % In-depth evaluation of individual component or property

==> eval.tex <==
\section{Evaluation}
\label{sect:eval}

We assess \name's overall merits for users and network ($\S$\ref{sect:eval:overall}),
and validate its properties for its key components ($\S$\ref{sect:eval:micro}).

\paragraphb{Prototype:}

\paragraphb{Dataset:}


\paragraphb{Experimental setup:}
\todo{Evaluation metrics, scenarios, baseline, and methodology. Would be nice if the evaluation can cover some use cases in $\S$\ref{sec:back:case}.}

\paragraphb{Ethical evaluation:} This work does not raise any ethical issues. %\yuanjie{mandatory according to SIGCOMM CFP}

\input{eval-overall} % End-to-end evaluation from user/network's perspective
\input{eval-micro}   % In-depth evaluation of individual component or property

==> impl.tex <==
\section{Implementation}
\label{sect:impl}

An IPv6-based implementation, but \name can also use other architecture (NDN \cite{zhang2014named,jacobson2009networking}, MobilityFirst \cite{mobilityfirst}, SCION \cite{zhang2011scion}, XIA \cite{han2012xia})

\paragraphb{\name construction:}

\paragraphb{\name address embedding:} How to encode location information into IPv6 headers (address, hop-by-hop header, prefix/suffix, \etc.)

\paragraphb{\name routing engine:} Quagga+LAP \lixin{Check in the details}

\paragraphb{Testbed:} \textsf{mininet} \lixin{Check in the details}


\iffalse
\paragraphb{Adopting \name in state-of-the-art IPv6:} Discuss the details of embedding our location addressing into IPv6 packet

\begin{compactitem}
\item Location in IPv6 source/destination address or optional extension header? How should the address or header look like?
\item Prefix and suffix design: DAD/RA, smart selection (be concise)
\item How many bits to be used?
\item The impact of area size
\item \todo{Should we discuss DNS?}
\end{compactitem}

\paragraphb{Adopting \name in ``future'' Internet architecture:} NDN, MobilityFirst, XIA, SCION
\fi




==> intro-v1.tex <==
\section{Introduction}
\label{sect:intro}

The future Internet is up in the sky. 
%Since 2019, we have witnessed 
Since 2019, we have witnessed a rocket-fast deployment of the low-earth-orbit (LEO) satellite mega-constellations for the Internet in space, including the SpaceX Starlink \cite{starlink}, Amazon Kuiper \cite{kuiper}, TeleSat \cite{telesat}, OneWeb \cite{oneweb}, to name a few. 
Compared to the traditional satellite networking at medium/high-earth orbit (MEO/HEO) orbits, 
these LEO mega-constellations promise ultra-low network latency and high throughput that are competitive to the terrestrial networks. %, and retains global Internet coverages to areas with limited terrestrial network infrastructure. 
Moreover, with thousands of LEO satellites, these mega-constellations retain the global Internet coverage to users that were not easily reachable by terrestrial networks, such as those in rural areas and ocean.

This work starts with a simple question: {\em How to enable effective and scalable inter-networking, addressing and routing for the Internet in space?}
%Despite diverse mega-constellations with numerous satellites today, existing designs (including 
Despite the rapid deployments of LEO mega-constellations, these industrial efforts's primary goal is to guarantee the {\em full coverage}. 
%It is until recently when SpaceX starts to recruit network engineers to build the networking technology for Starlink \cite{starlink-engineer}.
%Meanwhile, the research community has validated the potential performance gains of LEO mega-constellations in various aspects, such as the low network latency \cite{klenze2018networking, bhattacherjee2018gearing}, the acceleration of content delivery to ground stations \cite{handley2019using, quasar2021mobicom}, %bhattacherjee2019network}
%.
Meanwhile, the research community has validated on the potential network performance gains from LEO mega-constellations in various scenarios, such as low-latency networking \cite{handley2018delay, klenze2018networking, bhattacherjee2018gearing, handley2019using, bhattacherjee2019network}, in-orbit computing \cite{bhattacherjee2020orbit}, acceleration of content delivery for ground stations \cite{quasar2021mobicom, adrian2020backbone}, to name a few.
%\cite{klenze2018networking, bhattacherjee2018gearing, handley2019using, bhattacherjee2019network, bhattacherjee2020orbit}.
However, it is unclear {\em how} to realize these improvements with effective networking, addressing, and routing for mega-constellations. 
\yuanjie{BE CAREFUL with these statements. Avoid backfire by the community.}

A fundamental challenge for networking with LEO mega-constellations is to guarantee {\em stable network services at scale} ($\S$\ref{sec:challenge}).
With the high mobility of satellites and earth, networking with the existing mega-constellations suffers from three deficiencies of stability on the network and user\footnote{A ``user'' can be a satellite phone, a satellite dish, or a ground station.} sides:
\yuanjie{Shorten the challenges. Move most materials to $\S$\ref{sec:challenge}.}

\begin{compactenum}

\item {\em Unstable satellite network topology:}  Compared to the MEO/GEO satellites, LEO satellites at much lower altitude (typically $\leq$2,000 km) exhibit high mobility and relative motions.
This results in frequent satellite network topology and inter-satellite link (ISL) changes.
It not only complicates the network routing in space, but also triggers repetitive re-convergence in routing protocols and therefore significantly lowers the network usability ($\leq$10\% network availability for Starlink and Kuiper)\lixin{update the number}. 

\item {\em Unstable user addressing:} 
The classical logical network addressing suffers from frequent changes.
With rapid satellite motions, the terrestrial users served by one satellite have to frequently switch to new satellites (thus new network interfaces and address) to retain its Internet access. %(every 120--125s per user, and 1000--6000 IP address changes per second in Starlink). 
In Starlink, each user should change its logical IP address every 120--125s, and every 1000--6000 users per second should change their IP addresses as their serving satellites moves. 
%
Such frequent address changes will repetitively disrupt the TCP connections and upper-layer applications, thus negatively impacting the user experiences of satellite network services. 

\item {\em Unstable satellite-user mapping:}
The earth's rotation and its relative motion to satellites complicate the network routing. 
The satellite-user mapping is time-varying and highly dynamic: Each moving satellite serves more than one terrestrial user, while each user has choices of multiple access satellites each time. 
It is a challenging task to properly locate the satellite and terrestrial users for correct and efficient routing.

\end{compactenum}
%Even worse, the {\em mega}-constellations worsen all these stability issues, and 
%Even worse, all these stability issues can be amplified by more satellites in the {\em mega}-constellations. 
Moreover, all these stability issues are amplified as the {\em mega}-constellations scale to thousands of satellites. 
Solutions for small LEO networking 20 years ago (\eg, virtual topology \cite{werner1997dynamic, chang1998fsa} and virtual nodes \cite{ekici2000datagram, ekici2001distributed}) cannot scale to the mega-constellations today due to their high complexity. 

To this end, we propose \name (``Fractal Rosette''), a LEO mega-constellation for stable and scalable networking in space. 
For high scalability, \name defines a recursive interconnection structure over the Rosette constellation \cite{ballard1980rosette}. 
To stabilize the networking, \name adopts earth-repeat orbits over its LEO satellites to guarantee invariant logical network topology despite high mobility. 
To stabilize the user addressing, \name decouples the addressing from satellite/earth mobility via stable and hierarchical {\em geographical} address.
This is achieved by exploiting \name's recursive structure, and dividing the earth geometry into hierarchical cells by its earth-repeat orbits.
%To stabilize the users' address, \name assigns {\em geographical} network address to users by dividing the earth surface into stable and hierarchical cells by its earth-repeat orbits.
%\name divides the earth surface into stable and hierarchical geographical cells by its earth-repeat orbits, and allocates geographical network address to users.
In this way, \name also guarantees stable and predictable satellite-user mapping over time. 
\name provides local geographic routing with provably guaranteed delivery and bounded hops/delays, without requiring global routing convergence.  
%based on longest prefix matching and supports multi-path routing. 
For the resource-constrained satellites, \name can realize its location-based routing with readily-available, efficient longest prefix matching. 
\name also supports multi-path routing for high performance and fault tolerance, and on-demand incremental expansion with fewer satellites. 
%\name supports efficient single-path routing with bounded latency, multi-path routing for high performance and fault tolerance, and on-demand incremental expansion with fewer satellites.

We prototype \name's construction and routing over satellite routers, and evaluate it with trace-driven emulations. 
Compared to the state-of-the-art mega constellations (Starlink, Kuiper, and Iridium), \name can guarantee full coverage with XXX\% fewer satellites. \wei{Check in numbers}
Compared to existing LEO networks topology (motif \cite{bhattacherjee2019network}), \name achieves achieves XXX$\times$ higher service availability and XXX$\times$ less address changes\lixin{Check in numbers}. 
Meanwhile, \name incurs negligible system overhead for resource-constrained satellites, and marginal latency penalty for users. 

\iffalse
\todo{diff motif from stability. diff LEO networking 20 years ago from scalability perspective.}

Existing networking in LEO mega-constellations cannot meet the following properties simultaneously
\begin{compactenum}
\item Stable network topology in space; 
\item Stable geographical cells on earth surface; {\em and} 
\item Stable satellite-to-cell mapping (not necessarily 1-to-1; can be 1-to-many or many-to-1).
\end{compactenum}
Among them, Starlink and Kuiper also satisfy (1), Google S2 and Uber H3 also satisfy (2), and Geo-stationary satellite satisfies (3).
\fi


\iffalse
\p{``Stability'' in \name means 
\begin{compactenum}
\item Stable network topology in space; 
\item Stable geographical cells on earth surface; {\em and} 
\item Stable satellite-to-cell mapping (not necessarily 1-to-1; can be 1-to-many or many-to-1).
\end{compactenum}
Among them, Starlink and Kuiper also satisfy (1), Google S2 and Uber H3 also satisfy (2), and Geo-stationary satellite satisfies (3).
But {\bf no existing solutions can meet (1)--(3) \underline{\em simultaneously}.} 
}
\fi


%\name: Fractal rosette (cyclic recursion)


\iffalse

{
Location-based satellite networking and geographic addressing/routing were actively studied 20 years ago (mostly in the context of Iridium and terrestrial ad-hoc networks). Since then, however, modern satellite networking have been dramatically different from those 20 years ago, which invalidate old approaches and call for a {\bf totally new solution}:  

%Novelty of this work in terms of problem:

\begin{compactenum}

\item {\bf From GEO/MEO to LEO satellites:} For lower latency and higher throughput, modern satellite constellations widely adopt LEO satellites. However, this poses dramatic relative movement among satellites and terrestrial users, causing frequent IP address and network topology changes (thus re-convergence for link-state routing protocols and low availability);

\item {\bf From small to \underline{\em mega} constellation:} Two orders of magnitude more satellites than Iridium 20 years ago. This results in various implications for addressing:
	\begin{compactitem}
	\item {\em No one-to-one mapping:} Every terrestrial area is covered by more than one satellite, and every {\em fast-moving} satellite can cover more than one terrestrial cells. This invalidates the ``virtual node'' for Iridium 20 years ago, and challenges the {stability} of the user IP address and network topology; 
	\item {\em Multi-layer constellation:} Heterogeneous satellite orbits with diverse heights, inclinations, and launch time. This invalidates previous over-simplified solutions that assume homogeneous and polar orbits.
	\end{compactitem}
	
\item {\bf From terrestrial users to in-orbit computing:}
The convention satellite networking mainly serves terrestrial users only.
Until recently, the in-orbit computing is an appealing feature for many applications, such as CDN \cite{Amazon Kuiper}, secure storage \cite{XXX}, navigation \cite{XXX}, telemetry \cite{XXX}, Black Jack \cite{XXX}, to name a few. 
With in-orbit computing, both the terrestrial users and satellites will have layer-4 (and beyond) capabilities. 
To prevent service disruption, the addressing should be stable for both terrestrial users and satellites. 

\item {\bf From 2D to 3D spaces:} Most geographic routing solutions target 2D areas, using greedy routing for efficiency and planar (``face'') routing for loop-freedom. 
%Unfortunately, they are not applicable to 3D spaces in satellite networking.
However, location-based routing in 3D spaces is much harder than those in 2D spaces.
It has been recently proven that \cite{durocher2008routing}, {\em in general, no deterministic geographic routing algorithms in three-dimensional spaces can guarantee successful delivery of all packets to their destinations}. 
So it is open to question whether satellite networking in 3D spaces can bypass this limit, \eg, by exploiting it regular mobility pattern and orbit trajectories. 

\end{compactenum}}
\fi


==> intro-v2.tex <==
\section{Introduction}
\label{sect:intro}

The future Internet is up in the sky. 
%Since 2019, we have witnessed 
Since 2019, we have witnessed a rocket-fast deployment of the low-earth-orbit (LEO) satellite mega-constellations, including SpaceX Starlink \cite{starlink}, Amazon Kuiper \cite{kuiper}, TeleSat \cite{telesat}, OneWeb \cite{oneweb}, to name a few. 
Compared to the traditional satellite networking at medium/high-earth orbit (MEO/HEO) orbits, 
these LEO mega-constellations promise ultra-low network latency and high throughput that are competitive to the terrestrial networks. %, and retains global Internet coverages to areas with limited terrestrial network infrastructure. 
Moreover, with thousands of LEO satellites, these mega-constellations retain the global Internet coverage to users that were not easily reachable by terrestrial networks, such as those in rural areas and ocean.

This work starts with a simple question: {\em How to enable effective inter-networking in space to serve terrestrial users?}
Despite the rapid deployments of LEO mega-constellations, inter-connecting satellites for global network service is still at early trials and adoption. 
With numerous satellites in a highly dynamic and mobile environment, it is open to question whether traditional satellite and terrestrial networking design still fits for the LEO mega-constellations.



\iffalse
This work starts with a simple question: {\em How to enable effective and scalable inter-networking, addressing and routing for the Internet in space?}
%Despite diverse mega-constellations with numerous satellites today, existing designs (including 
Despite the rapid deployments of LEO mega-constellations, these industrial efforts's primary goal is to guarantee the {\em full coverage}. 
%It is until recently when SpaceX starts to recruit network engineers to build the networking technology for Starlink \cite{starlink-engineer}.
%Meanwhile, the research community has validated the potential performance gains of LEO mega-constellations in various aspects, such as the low network latency \cite{klenze2018networking, bhattacherjee2018gearing}, the acceleration of content delivery to ground stations \cite{handley2019using, quasar2021mobicom}, %bhattacherjee2019network}
%.
Meanwhile, the research community has validated on the potential network performance gains from LEO mega-constellations in various scenarios, such as low-latency networking \cite{handley2018delay, klenze2018networking, bhattacherjee2018gearing, handley2019using, bhattacherjee2019network}, in-orbit computing \cite{bhattacherjee2020orbit}, acceleration of content delivery for ground stations \cite{quasar2021mobicom, adrian2020backbone}, to name a few.
%\cite{klenze2018networking, bhattacherjee2018gearing, handley2019using, bhattacherjee2019network, bhattacherjee2020orbit}.
However, it is unclear {\em how} to realize these improvements with effective networking, addressing, and routing for mega-constellations. 
\yuanjie{BE CAREFUL with these statements. Avoid backfire by the community.}
\fi

A grand challenge for LEO satellite network is to guarantee {\em stable network services for terrestrial users at scale}.
Different from the traditional satellite network at high altitudes (\eg, geostationary communication satellites), LEO satellites exhibit high mobility and relative motions to the rotating earth.
%Under high relative motions between satellites and terrestrial users, traditional logical network design suffers from frequent network address changes (thus frequent user service disruption) and routing protocol re-convergence (thus low network service usability).
Consequently, the logical network topology between the satellites and ground suffers from repetitive changes, which results in frequent network address changes and routing protocol re-convergence.
Our analysis of existing mega-constellations in $\S$\ref{sec:challenge} shows that, with satellite mobility and earth's rotations, every terrestrial user switches his/her IP address every 120--125s (with 1,000-6,000 users/s changing IP addresses), and the satellite network usability decreases to $\leq$20\% due to frequent routing re-convergence.
%(every 120--125s per user, and every 1,000-6,000 users per second) and 
Moreover, these stability issues are amplified as the {\em mega}-constellations scale to thousands of satellites.
%Small LEO network designs 20 years ago cannot scale to the mega-constellations today due to their high complexity. 
%The fundamental problem is that, there exists a long-standing inconsistency between the {\em network design in cyberspace}, and the {\em addressing/routing in the physical world}.

\todo{Don't over-highlight ``unify virtual cyberspace and real physical world''. Highlight ``high dynamics'' (need a better term) between space and ground.}
The fundamental cause of the above unstable space-ground network is the mismatch between network in the {\em virtual cyberspace} and mega-constellation in the {\em physical world}.
On one hand, classical mega-constellations primarily focus on offering good coverage, but neglects the requirements from network addressing and routing. 
On the other hand, most (satellite) networks in the virtual cyberspace heavily rely on the logical address and routing, which are vulnerable to the high mobility of massive satellites and earth's rotations in reality.
A large-scale stable space-ground network calls for a consistent design of constellation, topology, addressing, and routing between cyberspace and reality.


\todo{Highlight stability under high dynamics. Highlight \name's friendliness to CPU/memory-constrained LEO satellites.}
%We propose \name\footnote{\name is short for ``Fractal Rosette''.}, an LEO mega-constellation for the stable space-ground network at scale. %between satellites and terrestrial users. 
We propose \name\footnote{\name is short for ``Fractal Rosette''.}, a stable space-ground network structure for the LEO satellite mega-constellation. 
\name aims to form a coherent time-space basis of network topology, addressing, and routing between the virtual cyberspace and the physical world.
It devises a recursive structure over the Rosette constellation \cite{ballard1980rosette} with earth-repeat orbits.
This structure ensures provably stable virtual network topology in the highly-mobile physical world, thus preventing routing re-convergence and retaining high network usability.
To stabilizes addressing in mobility, \name unifies the logical network address and geographical location, and derives hierarchical addresses for its users.
%This addressing scheme further enables stable and efficient routing.
This addressing further unifies and stabilizes the routing between satellites and terrestrial users. %in the graphical virtual topology and physical geographical locations.
%The geographical routing between terrestrial users can be embedded into the graphical routing between satellites.
Satellites run {\em local} prefix/wildcard match-based single/multi-path routing over the time-invariant network topology, without requiring global re-convergence.
To route traffic between terrestrial users, \name performs geographical routing by converting it into the topological routing between satellites.
%Geographical routing between terrestrial users can be converted to the topological routing between satellites for efficiency and stability.
%\name's routing is based on IPv6, and accelerated with readily-available prefix/wildcard matching in commodity routers.
%\name can be realized on top of IPv6 and accelerated with the readily-available prefix/wildcard matching. %in commodity routers.
\name can be efficiently realized with IPv6 for resource-constrained satellites, and incrementally expanded in practical deployments.
%\name supports IPv6-based implementation and incremental expansion. %and interconnection to external networks.

%This ensures time-invariant network address despite satellite mobility and earth's rotations.
%This structure enables stable and scalable logical network topology in the highly-mobile physical world.
%To stabilize the network addressing, \name defines  
\iffalse
To stabilize the networking, \name adopts earth-repeat orbits over its LEO satellites to guarantee invariant logical network topology despite high mobility. 
To stabilize the user addressing, \name decouples the addressing from satellite/earth mobility via stable and hierarchical {\em geographical} address.
This is achieved by exploiting \name's recursive structure, and dividing the earth geometry into hierarchical cells by its earth-repeat orbits.
%To stabilize the users' address, \name assigns {\em geographical} network address to users by dividing the earth surface into stable and hierarchical cells by its earth-repeat orbits.
%\name divides the earth surface into stable and hierarchical geographical cells by its earth-repeat orbits, and allocates geographical network address to users.
In this way, \name also guarantees stable and predictable satellite-user mapping over time. 
\name provides local geographic routing with provably guaranteed delivery and bounded hops/delays, without requiring global routing convergence.  
%based on longest prefix matching and supports multi-path routing. 
For the resource-constrained satellites, \name can realize its location-based routing with readily-available, efficient longest prefix matching. 
\name also supports multi-path routing for high performance and fault tolerance, and on-demand incremental expansion with fewer satellites. 
%\name supports efficient single-path routing with bounded latency, multi-path routing for high performance and fault tolerance, and on-demand incremental expansion with fewer satellites.
\fi

%We prototype \name's construction and routing over satellite routers, and evaluate it with trace-driven emulations. 
We prototype \name's protocol suite and evaluate it with hardware-in-the-loop, trace-driven emulations.
Compared to state-of-the-art mega constellations (Starlink, Kuiper, and Iridium), \name offers the same coverage with \del{at least }44\% fewer satellites. 
It stabilizes network topology, addressing, and routing with near-optimal data delivery. 
%Compared to existing LEO networks topology (motif \cite{bhattacherjee2019network}), \name achieves achieves XXX$\times$ higher service availability and XXX$\times$ less address changes\lixin{Check in numbers}. 
%Meanwhile, \name incurs negligible system overhead for resource-constrained satellites, and marginal latency penalty for users. 
Meanwhile, \name incurs negligible system overhead, thus suitable for resource-constrained LEO satellites.


==> intuition.tex <==
%\section{An Overview of \name}
\section{\name: Location-based Addressing}
\label{sec:intuition}
\label{sec:overview}

This section overviews \name, our addressing solution for integrated space-terrestrial networking.

\input{design-space}
\input{overview}

==> overview.tex <==
\subsection{An Overview of \name}
\label{sec:overview:overview}

==> practical-issues-v2.tex <==
\section{Issues in Practical Deployment}
\label{sec:deployment}

In this section, we discuss various issues and solutions for the deployment of \name in practice.

\yuanjie{Except \ref{sec:deployment:incremental}, other aspects are optional. Decide whether to include them based on space availability.}

\subsection{Incremental Expansion}
\label{sec:deployment:incremental}

\save{
\begin{figure}[t]
\subfloat[Hierarchical expansion]{
\includegraphics[width=0.59\columnwidth]{figures/hierarchical-deployment.pdf}
\label{fig:deployment:hierarchical}
}
\subfloat[Flat expansion]{
\includegraphics[width=0.41\columnwidth]{figures/flat-deployment.pdf}
\label{fig:deployment:flat}
}
\caption{Two incremental expansions in \name.}
\label{fig:deployment}
\end{figure}
}


In practice, it is unlikely to deploy \name all at once. The satellites can only be launched to space incrementally. 
For example, as of January 2021, the latest SpaceX Falcon 9 rocket can launch up to 143 satellites each time \cite{rocket-capability}, which is less than $\name_1$'s 256 satellites when $N=16$.
When incrementally expanding \name in space, it is desirable to retain always-on, seamless network services for existing users. 
This demand results in three concrete goals in expansion: (1) guarantee data delivery despite incomplete deployment; (2) avoid re-interconnection of satellites whenever possible; and (3) retain stable address during the deployment. 
\save{To this end, we devise two incremental expansion approaches for \name (exemplified in Figure~\ref{fig:deployment}): A recursive {\em hierarchical deployment}, and an iterative {\em flat deployment}.


\paragraphb{Recursive hierarchical expansion:}
The recursive construction of \name in Algorithm~\ref{algo:construction} implies a natural hierarchical expansion: Deploy $\name_{k-1}$ at higher altitude first, and then use it as a {\em backbone} to connect satellites in $\name_{k}$ at lower altitude. 
When $\name_k$ is being expanded, the high-altitude $\name_{k-1}$ guarantees full coverage (thus successful data delivery) to all terrestrial users.
Moreover, to ensure $\name_k$'s successful routing before its full deployment, each satellite $i$ in the high-altitude $\name_{k-1}$ connects to its corresponding satellites at lower altitude according to Algorithm~\ref{algo:construction}. 
In this way, if two lower-altitude satellites in $\name_{k-1}$ are unreachable due to incomplete deployment, their packets can always routed to their corresponding higher-altitude satellites in $\name_k$ for guaranteed delivery.
During this expansion, all satellites' addresses remain the same as those in $\S$\ref{sec:address:sat}.
%Note that satellites at different altitudes move at different speed, thus causing relative motions.


One issue for the hierarchical deployment is to coordinate the altitudes of satellites in $\name_{k-1}$ and $\name_k$. 
Note that satellites at different altitudes have different orbital periods.
To ensure the hierarchical geographical cell divisions in $\S$\ref{sec:address}. the orbit periods of $\name_{k-1}$ and $\name_k$ should satisfy  $T_{k-1}=NT_k$.
According to the Kepler's third law $T_{k-1}^2/(R_{k-1}+R_E)^3=T_{k}^2/(R_{k}+R_E)^3$, the altitudes should satisfy 
$\frac{R_{k-1}+R_E}{R_{k}+R_E}=N^{\frac{2}{3}}$.

Although hierarchical expansion is straightforward for incremental deployment, it requires additional satellites at higher altitudes besides the original \name construction (\eg, 8+64 satellites for $\name_1$ when $N=8$). 
%Each large cell will be divided into $a^2$ small cells. In order to meet this feature, it is necessary to control the satellite sub-point trajectory of  $\name_k$ to pass through all the intersections of the sub-satellite point trajectories of  $\name_{k-1}$. It can only work when $a$ is an integer. At the same time, the movement direction of the satellites belong to $\name_k$ and $\name_{k-1}$ at the intersections should be consistent, so $a$ needs to be an odd integer.
We next explore whether incremental expansion is possible at the same altitude. }


%Deploy $\name_{k-1}$ first at higher altitude, and then expand it to $\name_k$ at lower altitude. 
%In this process, the high-altitude $\name_{k-1}$ guarantees full coverage to all terrestrial users, and plays as a {\em backbone} to interconnect low-altitude satellites in $\name_k$ before the full deployment. 

%\paragraphb{Iterative flat expansion:}
%When incrementally expanding \name at the same altitude, 
%To this end, we devise an incremental expansion approaches for \name.
A straightforward way to incrementally deploy \name is to follow Algorithm~\ref{algo:construction}, \ie, launch $\name_{k-1}$ first and recursively expand it to $\name_{k}$. 
This ensures stable network topology and addresses, but can't guarantee delivery with partial coverage {\em before} all satellites are launched ($\S$\ref{sec:construction}). 
%The main challenge is to guarantee data delivery {\em before} all satellites are deployed. 
%As explained in $\S$\ref{sec:construction} and exemplified in Table~\ref{tab:altitude}, before all satellites are available, \name will not ensure full coverage at the minimal altitude. 
%If the same recursive expansion in Algorithm~\ref{sec:construction} is used at the same altitude, a single $\name_{k-1}$ at lower altitude cannot guarantee full coverage. 
%The users outside the the coverage cannot send or receive data. 

To this end, we propose an iterative incremental expansion scheme, and exploit regular satellite mobility to guarantee the data delivery. %of delay-tolerant data. 
Instead of building $\name_k$ from $\name_{k-1}$, we incrementally deploy it {\em orbit by orbit}.
Following step 8--12 in Algorithm~\ref{algo:construction}, each time we deploy satellites that uniformly distribute on the same orbit. %\fixme{How many satellites? How many times?}.
As exemplified in Figure~\ref{fig:iterative-expansion}, \name satellites in the same orbit form a moving wave of satellite sub-point trajectories that traverse the entire coverage. 
This differs from the satellite sub-points in a complete $\name_{k-1}$, which are fixed and thus limit its full coverage at lower altitude. 
As the satellite sub-point trajectories move, all users have the opportunity to send the data to the satellite sometime. 
If a packet's destination is currently outside the coverage, it can be buffered by the satellite and eventually delivered if any one of the satellite on the same orbit covers the destination. 
With more satellites deployed, more packets will be delivered via routing and less packets will be buffered. 
Similar to DTN in classical satellite networking~\cite{cerf2007delay, burleigh2003delay}, this approach is feasible when the \name users are all tolerant to data delays. 

\begin{figure}[t]
\vspace{-10mm}
\subfloat[$t=0$]{
%\includegraphics[width=0.5\columnwidth]{figures/incremental-expansion-1.pdf}
\includegraphics[width=0.5\columnwidth]{figures/incremental-expansion-1-v3.pdf}
\label{fig:deployment:t0}
}
\subfloat[$t=T/N$]{
%\includegraphics[width=0.5\columnwidth]{figures/incremental-expansion-2.pdf}
\includegraphics[width=0.5\columnwidth]{figures/incremental-expansion-2-v3.pdf}
\label{fig:deployment:t1}
}
\vspace{-2mm}
\caption{Exploiting regular satellite mobility to guarantee data delivery in flat incremental expansion.}
\label{fig:iterative-expansion}
\end{figure}

\iffalse
\subsubsection{Two Physical Deployment Scenarios}

\begin{compactitem}

\item {\bf Flat realization:} All satellites reside at the same altitudes. This approaches do not need high-altitude satellites, thus shorter ground-to-satellite RTT. But it is not friendly to incremental expansion\yuanjie{Really?}: All satellites should be available before enabling $\name_k$. Besides, detouring can happen (see Theorem~\ref{thm:hop}--\ref{thm:latency}).

\item {\bf Layered realization:} $\name_{k-1}$ as MEO (Backbone), and $\name_k$ as LEO (access network). The backbone $\name_{k-1}$ at higher altitude connects all $\name_k$ at lower altitude. This facilitates incremental expansion, and mitigates the detouring inc(to be detailed in $\S$\ref{sec:routing-sat}).
\wei{How to choose the altitude (or $T_s$) between $\name_{k-1}$ and $\name_k$, such that the topology remains stable despite their differences of altitudes and orbital periods? Draft:To satisfiy the feature that the cells of  $\name_{k-1}$ can be divided into cells of $\name_k$, the periodic relationship between them is  $T^{k-1}_s=aT^{k}_s$, where $a$ is an odd integer.Each large cell will be divided into $a^2$ small cells. In order to meet this feature, it is necessary to control the satellite sub-point trajectory of  $\name_k$ to pass through all the intersections of the sub-satellite point trajectories of  $\name_{k-1}$. It can only work when $a$ is an integer. At the same time,the movement direction of the satellites belong to $\name_k$ and $\name_{k-1}$ at the intersections should be consistent, so $a$ needs to be an odd integer.}
\end{compactitem}


\subsubsection{On-Demand, Incremental Expansion}

\subsubsection{Partial \name Deployment}
\fi



\subsection{Implications for Ground Stations}

The ground stations can play as ``gateways'' to bridge the satellite and terrestrial networks, or download telemetry data from satellites \cite{aws-gs,ms-gs,quasar2021mobicom, adrian2020backbone}.  
%It is also widely deployed to download massive data from LEO satellites for earth observations. 
It is desirable to deploy the ground stations where they can maximize its radio quality and access to more satellites.  
\name's stable satellite-to-ground mapping offers a natural solution for this.
A ground station using \name can be deployed at the intersection of the fixed satellite sub-point trajectories.
This guarantees maximal received power from the satellites (right above the ground station), and helps gain visibility to more satellites. 
%\fixme{Refine the deployment strategy. }
\yuanjie{Highlight stability in incremental expansion: No link or address change.}

%Deploy the ground station along the trajectory of satellite sub-point. 

\iffalse
\subsection{Fault Tolerance}

\name is resilient to network failures with its built-in multi-path routing. 
In presence of a satellite/ISL failures, \name can adapt its single-path routing in Algorithm~\ref{algo:single-path-routing} to bypass the failures.
Specifically, \name can permute the ordering of its address to iterate in Algorithm~\ref{algo:single-path-routing}, and build an alternative path to work around the failed satellite or link. 
\yuanjie{Elaborate on how to detect failures, and how to coordinate satellites to bypass the failures {\em without} requiring global convergence.}
\fi

\subsection{Network Address Allocation}
For satellites, their \name addresses in $\S$\ref{sec:address:sat} are fixed and can be pre-allocated before they are launched.
For the ground users, their \name addresses in $\S$\ref{sec:address:ue} are fixed unless they move to a new geographical cell. 
To tackle it, a DHCP address server (\eg, at the ground station) can be deployed for each cell to manage the address allocation and duplication detection.
As evidenced in Figure~\ref{fig:user-address}, the DHCP server can generate a \name address by concatenating the network prefix, the geographical cell ID, and a per-user suffix that is unique inside this cell.

\subsection{Inter-networking to External Networks}
\label{sec:discuss:external}

The discussion so far focuses on the networking inside a \name. 
In reality, both the terrestrial users and satellites need to communicate with others through the Internet. 
For compatibility with Internet routing and global reachability, we propose IPv6-based network addressing for \name. 
As shown in $\S$\ref{sec:address} and exemplified in Figure~\ref{fig:address}, %both the satellite and terrestrial user's hierarchical addresses in \name can be directly embedded into an IPv6 address. 
the IPv6 prefix in Figure~\ref{fig:user-address} can be used to identify whether a packet is inside a \name. 
If so, the \name routing in $\S$\ref{sec:routing} can be applied.
Otherwise, the packet will leave \name and enter the external network.
In this case, the classical prefix match-based IP routing will be applied to the IPv6 address, thus retaining backward compatibility and global reachability. 

\subsection{Stability-Performance Tradeoff}
\label{sec:discuss:tradeoff}

%The \name design prioritizes stability to performance for a usable space-ground network.
\name's primarily goal is to ensure stability for a usable space-ground network.
It is possible to refine \name to balance the stability and performance.
For instance, the basic \name design only utilizes local links to guarantee the stable network topology (Theorem~\ref{thm:stability}). 
It is possible to extend \name with non-local links for lower latency (first proposed in \cite{bhattacherjee2019network}), by using a base Rosette constellation in Figure~\ref{fig:base-case} and recursive construction in Algorithm~\ref{algo:construction} with $m$-local links.
In this case, the maximum number of hops in Theorem~\ref{thm:hop} can be reduced to $\frac{N(k+1)}{2m}$.
The cost is the potential link failures (Theorem~\ref{thm:stability}) and unstable routing.
We leave the comprehensive study of this tradeoff for the future work.
%We are neutral to this tradeoff and leave it for the operators to decide based on their demands.

\iffalse
For stability, the basic \name design only utilizes local links for networking in space. 
Recent work \cite{bhattacherjee2019network} has demonstrated that, it is possible to establish ISLs between {\em non-local} satellites for networking with lower latency. 
%The corresponding networking design, \textsf{motif}, offers near-optimal latency and $2\times$ throughput improvement. 
\name can support the same design by adding non-local ISLs in the base case in Figure~\ref{fig:base-case}.
The recursive construction in Algorithm~\ref{algo:construction}, while the single-path routing in Algorithm~\ref{algo:single-path-routing} should be extended to explore shorter non-local links (\ie, increasing the satellite addressing by more than 1).
The potential cost would be the risk of more failures for non-local ISLs, as quantified in Figure~\ref{fig:usability}. 
%We are neutral to these choices, and leave the freedom of using non-local ISLs to \name users. 

Note this bound can be further shortened by choosing the base case of \name with {\em non-local} links, similar to \textsf{motif} in \cite{bhattacherjee2019network}. 
With $m$-local links in $\name_k$, the maximum number of hops can be bounded by $\frac{N(k+1)}{2m}$.
The cost, however, is the potential failures to establish the inter-satellite links and thus routing failures.
We will discuss this in $\S$\ref{sec:discuss:tradeoff}. 
\fi


==> practical-issues.tex <==
\section{Issues in Practical Deployment}
\label{sec:deployment}

We discuss various issues and solutions for the deployment of \name in practice.

\subsection{Two Physical Deployment Scenarios}

\begin{compactitem}

\item {\bf Flat realization:} All satellites reside at the same altitudes. This approaches do not need high-altitude satellites, thus shorter ground-to-satellite RTT. But it is not friendly to incremental expansion\yuanjie{Really?}: All satellites should be available before enabling $\name_k$. Besides, detouring can happen (see Theorem~\ref{thm:hop}--\ref{thm:latency}).

\item {\bf Layered realization:} $\name_{k-1}$ as MEO (Backbone), and $\name_k$ as LEO (access network). The backbone $\name_{k-1}$ at higher altitude connects all $\name_k$ at lower altitude. This facilitates incremental expansion, and mitigates the detouring inc(to be detailed in $\S$\ref{sec:routing-sat}).
\wei{How to choose the altitude (or $T_s$) between $\name_{k-1}$ and $\name_k$, such that the topology remains stable despite their differences of altitudes and orbital periods? Draft:To satisfiy the feature that the cells of  $\name_{k-1}$ can be divided into cells of $\name_k$, the periodic relationship between them is  $T^{k-1}_s=aT^{k}_s$, where $a$ is an odd integer.Each large cell will be divided into $a^2$ small cells. In order to meet this feature, it is necessary to control the satellite sub-point trajectory of  $\name_k$ to pass through all the intersections of the sub-satellite point trajectories of  $\name_{k-1}$. It can only work when $a$ is an integer. At the same time,the movement direction of the satellites belong to $\name_k$ and $\name_{k-1}$ at the intersections should be consistent, so $a$ needs to be an odd integer.}
\end{compactitem}


\subsection{On-Demand, Incremental Expansion}

\subsection{Partial \name Deployment}

\subsection{Fault Tolerance}

Overall: Leverage redundant paths to tolerate failures, while still keeping the stable topology.

\paragraphb{Intermittent link failure:} due to radio fluctuations (most likely for microwave)

\paragraphb{Satellite failure:} Use backup satellites. At least $2V+3$ satellites for worldwide V-satellite visibility anywhere. 

\subsection{Implications for Ground Stations}

Deploy the ground station along the trajectory of satellite sub-point. 

\subsection{Re-structing Existing Constellations as \name}

\fixme{Potential counter arguments: ``Starlink has been launched. Why bother launching a new one? Why not optimize existing ones?''}

\yuanjie{Would it be possible to {\em re-struct} Starlink, Kuiper, OneWeb, \etc, such that they can be converted to a \name constellation? This way, we don't have to launch new constellations. Instead, existing ones can readily enjoy the benefits of stable routing from \name. Here ``re-struct'' can be (1) change the orbits and ISLs of existing satellites; (2) change the launch plan for the remaining satellites.}

==> problem-formulation.tex <==
\subsection{Problem Statement}
\label{sec:problem:formulation}

%\fixme{``integrated'' is thought as ``incremental work'' from SIGCOMM community. Any better word?}

We look for a new addressing scheme that is suitable for the integrated space-terrestrial network.
We assume XXX.
We seek a scheme that satisfies the following properties:
\todo{Definition, then explain why it matters for our scenario.}
\begin{compactitem}
\item {\bf Universal for territory and space:} Beneficial for inter-networking; simple for recent proposals of using ground stations for satellite routing [HotNets'19]. \todo{Lixin, can you provide some quantitive evidences from our testbed to support it?}
\item {\bf Locality:} If the addresses of two locations are close, their physical locations should also be close (and vice versa). This ensures the consistency between the digital and physical spaces, and facilitates the location-based routing. 
\item {\bf Stability:} The address of terrestrial and space nodes should remain invariant in presence of high mobility. This property seeks to minimize the disruptions of upper-layer applications, and the stability of the routing paths.
\item {\bf Clustering:} The addresses of physically close locations can be grouped with same prefix. This property facilitates the scalable routing in space and territory, similar to CIDA for IP address. 
\item {\bf Efficiency:} Processing the address should be fast enough, and consume as little resource as possible. This is crucial for resource-constrained satellites. 
\end{compactitem}

==> problem.tex <==
\section{Why New Addressing?}
\label{sec:problem}

This section explains why we need a new addressing for the network in space. 
We are aware that changing the addressing scheme would have a fundamental impact on the Internet architecture. 
In this section, we will explain why we {\em have to} do so, and what we demand for a new addressing scheme.

\input{address-impact}
\input{empirical-study}
\input{state-of-the-art}
\input{problem-formulation}







==> properties.tex <==
\subsection{Basic Properties of \name}

%\paragraphb{Number of satellites:} $N^{k+1}$ for $\name_k (k=0,1,...)$

%\paragraphb{Number of inter-satellite links:} 

\name inherits all good properties from the classical Rosette constellation in $\S$\ref{sec:rosette-primer}, and has additional appealing features for networking due to its recursive architecture. 

\paragraphb{Full coverage:} Each $\name_k$ is also a Rosette constellation, thus ensuring full coverage with fewer satellites as explained in $\S$\ref{sec:rosette-primer}.
Table~\ref{XXX} compares the number of satellites needed for full coverage by Starlink, Kuiper, and \name\lixin{Add the table. Compare \name with state-of-the-arts (Starlink, Kuiper, OneWeb, \etc) \wrt no. satellites, stability, scalability, routing, \etc. }. 
It shows that, at the same altitude and elevation angle, \name requires less satellites than state-of-the-art commercial constellations. 

\paragraphb{Stable and periodic satellite sub-point trajectory:} \name always adopts Rosette constellations with earth-repeat orbits $T_s=T_E/(P-m)$.
As shown in Figure~\ref{fig:construction:cell}, this results in earth-repeat orbits, thus stable and periodic satellite sub-point trajectory trajectories.
As we will see in $\S$\ref{sec:address}, this feature enables hierarchical and stable address for satellites and terrestrial users, and simplifies the routing in such a highly mobile environment. 



\paragraphb{Stable network topology:} A grand challenge for LEO networking is the high mobility among satellites, and between the satellite and earth. 
As shown in $\S$\ref{sec:challenge}, such high relative movement results in frequent re-routing and therefore low network service availability, and can be amplified with more satellites in the mega-constellation. 
Instead, \name prevents this by retaining a stable network topology.
\name interconnects the satellites with its local neighbors only, thus resulting in short yet stable ISLs.
As long as the altitude of a $\name_k$ is beyond the minimum altitude in $\S$\ref{sec:construction}, all connected satellites are visible to each other and maintain regular distance in Equation~\ref{eqn:isl-distance}.
This results in always-on, invariant inter-satellite links despite movement and earth rotation. 
%All links in $\name_k$ can be always-on despite satellite movement and earth rotation.

\iffalse
Specifically, we have the following theorem (proved in Appendix~\ref{proof:stability}):
\begin{thm}[Stable network topology]
%All links in $\name_k$ can be always-on despite satellite movement and earth rotation.
The graphical topology of a $\name_k$ remains invariant despite the time-varying satellite movement and earth rotation.
\label{thm:stability}
\end{thm}
\fi

\paragraphb{Regular inter-satellite link variation:}
%Although every inter-satellite link in $\name_k$ remains always on, 
The length of an inter-satellite link (thus propagation delay) varies over time regularly due to satellite mobility. 
For any two satellites $i$ and $j$, its inter-satellite link length $L_{ij}$ and propagation delay $T_{ij}$ are
\begin{align}
\label{eqn:isl-distance}
L_{ij} &=2\left ( H+R_{E} \right )\sin\left ( r_{ij}/2 \right ) \\
T_{ij} &=L_{ij}/c
\end{align}
%The inter-satellite {\em range} between $i$ amd $j$ is \lixin{propagation speed between satellites is equal to the speed of light c, thus the propagation delay is}
where $r_{ij}$ is the {\em range} between $i$ amd $j$ on the great circle:
\begin{align*}
\sin^2(r_{ij}/2) &= \cos^4(\beta/2)\sin^2(m+1)(j-i)(\pi/P)\\
		      &+ 2\sin^2(\beta/2)\cos^2(\beta/2)\sin^2m(j-i)(\pi/P)\\
		      &+ \sin^4(\beta/2)\sin^2(m-1)(j-i)(\pi/P)\\
		      &+ 2\sin^2(\beta/2)\cos^2(\beta/2)\sin^2(j-i)(\pi/P)\\
		      &\cdot\cos[2x+2m(j+i)(\pi/P)]\\ 
\end{align*}
Figure~\ref{fig:length_change} exemplifies the variance of link RTT between two satellites in $\name_1$. \lixin{Which 2 satellites?}
It confirms the predictive variance of the RTT, which is feasible for low-jitter applications. 
\yuanjie{With multi-hop routing, can we get even more stable RTT?}

\begin{figure}[t]
\includegraphics[width=\columnwidth]{figures/length_change.eps}
\caption{Variation of a satellite ISL in $\name_1$.}
\label{fig:length_change}
\end{figure}

\iffalse
\begin{align*}
	length=2\left ( H+R_{E} \right )sin\left ( r_{ij}/2R_{E} \right ) 
\end{align*}
\begin{align*}
	delay &= length/c\\
	     &=2\left ( H+R_{E} \right )sin\left ( r_{ij}/2R_{E} \right )/c\\   
\end{align*}
\fi

%Facilitate routing

\iffalse
\begin{compactitem}
\item {\em Stable topology:}
\item {\em Stable addressing:}
\end{compactitem}
\fi

%\paragraphb{Locality:}

%\paragraphb{Hierarchy:}



==> related.tex <==
\section{Related Work}
\label{sect:related}

\yuanjie{Tune the tone. The current writing is arrogant...}

Satellite constellation design has been an active research area since 1970s. 
Most work primarily focuses on ensuring satisfactory satellite coverage under various conditions, including the classical Walker constellation \cite{walker1984walker}, Rider constellation \cite{rider1986analytic}, Rosette constellation \cite{ballard1980rosette}, Ellipso \cite{castiel1995ellipso}, polar orbits \cite{tan2019new}, to name a few. 
The recent mega-constellations for LEO networking, such as Starlink \cite{sayin2019passive}, Kuiper \cite{boyle2019amazon}, Telesat \cite{telesat} and OneWeb \cite{oneweb}, largely inherit this design and prioritize coverage over networking. 
While +Grid and motif \cite{bhattacherjee2019network} seek to refine the network topology on top of these constellations, our study shows these efforts are insufficient to ensure fundamentally stable and scalable satellite networking. 
Instead, \name revisits the constellation design from the networking perspective, and provides an orthogonal approach for stable networking in space at scale.

\name belongs to the broader context of satellite networking design, which is at the renaissance with the recent proliferation of LEO mega-constellation. 
The early research on satellite networking explored various routing techniques, such as the addressing for terrestrial users \cite{alex2016addressing, preston2001geo, megen2001mapping, hain2002ipv6} and satellites \cite{hybridaddressing, walkeraddress}, virtual node \cite{ekici2000datagram, ekici2001distributed}, virtual topology {\cite{werner1997dynamic, chang1998fsa}}, multi-layer routing \cite{chen2005routing, lee2000satellite}, geographical routing \cite{lam2011geographic, kleinberg2007geographic, rao2003geographic, karp2000gpsr}. 
However, these efforts implicitly assume small constellations like Iridium~\cite{tan2019new} in 2000s, and do not scale to mega-constellations today due to their high complexity. 
%Instead, \name is designed for mega-constellations. 
\name is inspired by them but designed for mega-constellations. 
The recent work has taken the first step to validate the benefits of LEO mega-constellations, including the low-latency networking \cite{klenze2018networking, bhattacherjee2018gearing, handley2019using, bhattacherjee2019network}, in-orbit computing \cite{bhattacherjee2020orbit}, acceleration of content delivery for ground stations \cite{quasar2021mobicom, adrian2020backbone}, to name a few.
\name is orthogonal to these efforts. 
It takes one step further to study the stable and scalable network topology, addressing, and routing in mega-constellations. 
%\jiayi{\del{Also fill out the missing references below. }}

\todo{Comment on \name's distant similarity and difference from Hypercube and BCube in DCN.}
 
%\jiayi{\del{Survey all SIGCOMM TPC members at \url{http://conferences.sigcomm.org/sigcomm/2021/tpc.html}. Check if they have published any papers about satellites. If yes, cite them here.}}

\iffalse
\begin{compactitem}
\item Satellite constellation: Rosette constellation \cite{ballard1980rosette}, Walker constellation \add{\cite{walker1984walker}}, motif \cite{bhattacherjee2019network}, Starlink \add{\cite{sayin2019passive}}, OneWeb \add{\cite{radtke2017interactions}}, Kuiper \add{\cite{boyle2019amazon}}, TeleSat \add{\cite{telesat}}, Iridium \add{\cite{tan2019new}}
\item Satellite routing: Virtual node \cite{ekici2000datagram, ekici2001distributed}, virtual topology \add{\cite{werner1997dynamic, chang1998fsa}}, OSPF+/BGP+ \add{\cite{xu2017intra, wang2018bgp}}, routing for low latency \cite{handley2018delay, bhattacherjee2018gearing, klenze2018networking}, ground-station assisted \cite{handley2019using}, \add{CDN-like SN integration system \cite{adrian2020backbone}}
\item Usage scenarios: In-orbit computing \cite{bhattacherjee2020orbit}, observation satellites \cite{vasisht2020distributed}, in-flight Internet \cite{rula2016ips, rula2018mile}

\item Location-based routing: \jiayi{\del{Check in your previous survey results here, including each paper/patent's bib file (from Google Scholar, in English). }} \add{2D \cite{kleinberg2007geographic, ruehrup2009theory, stojmenovic2001loop}, 3D and higher dimensions \cite{lam2011geographic, flury2008randomized, durocher2008routing}} 

\item \name is inspired by BCube \cite{guo2009bcube}, DCell \cite{guo2008dcell} in data center networking and Chord \cite{stoica2001chord} in P2P.
\add{\item IP Addressing: Address only the surface \cite{alex2016addressing, preston2001geo, megen2001mapping, hain2002ipv6}, simultaneous surface and satellite addressing \cite{hybridaddressing, walkeraddress}}
\end{compactitem}
\fi




==> rosette-primer.tex <==
\subsection{A Primer of Rosette Constellation}
\label{sec:rosette-primer}

The basic building block of \name is a Rosette constellation, which was originally proposed in \cite{ballard1980rosette} to guarantee full coverage with as few satellites as possible.
This section introduces the necessary background of Rosette constellation for \name; a complete description is available in \cite{ballard1980rosette}.

Figure~\ref{fig:rosette-example} exemplifies the Rosette constellation with 8 satellites. %\wei{Add the figure}. 
All satellites move in circular orbits %\footnote{In general, the orbit of a satellite is elliptical according to Kepler's first law. But for a LEO satellite, its orbit's eccentricity is close to 0 ($\leq$0.001 for Starlink, Kuiper and Telesat according to the public orbital dataset \cite{space-track}\jiayi{add FCC citations} and thus can be approximated as a circular orbit.} 
at the altitude of $H_s$ (thus period $T_s$).
A Rosette constellation is defined as a parameter tuple $(N, P, m)$, where $N$ is the total number of satellites, $P$ is the number of orbits, $Q=N/P$ is the number of satellites per orbit, and $m$ is a harmonic phase shift factor.
All satellites are numbered from 0 to $N-1$.
For satellite $i$, its runtime location can be described by three constant angles $(\alpha_i,\beta_i,\gamma_i)$ and one time-varying phase angle $x_t$ at time $t$:

%\paragraphb{Construction:} A $N$-satellite Rosette constellation $(P, Q, m)$ ($N=PQ$) is constructed as follows:

\begin{align}
\alpha_i &= \frac{2\pi i}{P}, i=0,1,...,N-1 \label{eqn:alpha}\\
\beta_i &\equiv \beta, \forall i \label{eqn:beta}\\
\gamma_i &= m\alpha_i=mQ\cdot\frac{2\pi i}{N}, \hfill m\in[0,\frac{N-1}{Q}] \label{eqn:gamma}\\
x_t &= \frac{2\pi}{T_s}t \label{eqn:x}
\end{align}
where $\alpha_i$ is satellite $i$'s right ascension angle, $\beta_i\equiv\beta$ is the inclination angle for all orbits, $\gamma_i$ is $i$'s initial phase angle in its orbit at time $t=0$, and $x_t$ is the time-varying phase angle ({\em identical for all satellites anytime}). 
Compared to other constellations, the Rosette constellation has two appealing properties for networking:

\begin{figure}[t]
\vspace{-5mm}
\subfloat[Physical constellation in space]{
\includegraphics[width=0.5\columnwidth]{figures/rosette.pdf}
\label{fig:rosette-constellation}
}
\subfloat[Logical topology in $\name_0$ \todo{Clarify local connection is {\em NOT} the only choice for \name.}]{
\includegraphics[width=0.5\columnwidth]{figures/base-case.pdf}
\label{fig:base-case}
}
\vspace{-2mm}
\caption{An $(8,8,6)$ Rosette constellation.}
\label{fig:rosette-example}
\end{figure}

\iffalse
\begin{figure}[t]
\begin{minipage}{0.49\columnwidth}
\includegraphics[width=\columnwidth]{figures/3D-view.pdf}
\caption{\name in space.}
\end{minipage}
\begin{minipage}{0.49\columnwidth}
\includegraphics[width=\columnwidth]{figures/3D-view.pdf}
\caption{The \textsf{Rotation} operation in \name construction.}
\end{minipage}
\end{figure}
\fi



\paragraphb{Full coverage with fewer satellites:} 
%\name can fully cover the earth with at least 5 satellites at the altitude of 27,629 km (4.2$\times$ of earth radius). 
The Rosette usually needs fewer satellites than the Walker constellation (building block for Starlink and Kuiper) to ensure full coverage (see $\S$\ref{sec:eval:characteristics} for the evaluations). 
As shown in Figure~\ref{fig:coverage}, each satellite's coverage $R$  (in the earth's great circle range) can be determined by its altitude $H$ and elevation angle $\phi$:
\begin{equation}
\tan\phi=\frac{\cos R-R_E/(R_E+H)}{\sin R}
\label{eqn:altitude}
\end{equation}

For LEO satellites, given each satellite's coverage $R$ on the earth, the minimum number of satellites $N_{min}$ needed to fully cover the earth is decided by the following relation:

\begin{equation}
\sec R=\sqrt{3}\tan{\left(\frac{\pi}{6}\frac{N_{min}}{N_{min}-2}\right)}
\label{eqn:per-sate-coverage}
\end{equation}

\paragraphb{Stable, periodic ground-track repeat orbits:} Due to the earth rotation and high LEO satellite mobility, the satellite sub-point (Figure~\ref{fig:coverage}) is time-varying and non-repeatable in general\footnote{The geostationary satellites guarantee time-invariant satellite sub-point, but at the altitude of 35,786km and thus suffer from long network latency.}. 
This complicates locating and routing between the ground and space. 
Instead, the Rosette constellation allows LEO satellites to retain periodic satellite sub-points via ground-track repeat orbits, \ie, every satellite will {\em periodically} revisit its previous satellite sub-point. 
To do so, we configure the satellites' orbital period $T_s$ such that 
\begin{equation}
T_s=T_E/(P-m)
\label{eqn:repeat-orbit}
\end{equation}
where $T_E$ is the period of earth rotation. Then for each satellite $i$, the latitude $\phi_i$ and longitude $\lambda_i$ of its satellite sub-point varies periodically:
\begin{align}
&\sin\varphi_i = -\sin\beta\sin{m(\omega_Et-\alpha_i)} \label{eqn:phi}\\
&\tan{\left[\lambda_i+m(\omega_Et-\alpha_i)\right]}=-\cos\beta\tan m(\omega_Et-\alpha_i) \label{eqn:lambda}
\end{align}
where $\omega_E=2\pi/T_E$ is the earth's angular rotation speed.

\medskip
Despite these merits, however, the original Rosette constellation is not immediately applicable to networking. 
It was primarily designed for ensuring full coverage, not routing. 
There was no specification on how to inter-connect satellites, how to forward traffic among satellites, and how to route data among terrestrial users via satellites. 
This motivates us to move beyond coverage, and re-struct the Rosette constellation for scalable and stable networking in space. 



\iffalse
\paragraphb{Properties:}

\begin{compactenum}
\item {\em Full coverage:} By minimax satellite coverage, Rosette constellation can cover the earth with $\geq$5 satellites

The inter-satellite {\em range} between $i$ amd $j$ is \lixin{What's the ISL {\em length} (thus propagation delay)?}
\begin{align*}
\sin^2(r_{ij}/2) &= \cos^4(\beta/2)\sin^2(m+1)(j-i)(\pi/P)\\
		      &+ 2\sin^2(\beta/2)\cos^2(\beta/2)\sin^2m(j-i)(\pi/P)\\
		      &+ \sin^4(\beta/2)\sin^2(m-1)(j-i)(\pi/P)\\
		      &+ 2\sin^2(\beta/2)\cos^2(\beta/2)\sin^2(j-i)(\pi/P)\\
		      &\cdot\cos[2x+2m(j+i)(\pi/P)]\\ 
\end{align*}

\item {\em Fixed ground track orbits:} 
        $$\sin\varphi_i = \sin\beta\sin{m(\omega_Et+\alpha_i)}$$
        $$\tan{\left[\lambda_i+m(\omega_Et+\alpha_i)\right]}=\cos\beta\tan m(\omega_Et+\alpha_i)$$
        $$T_s=T_E/(P-m)$$
\item {\em The number of satellites needed:} %\todo{Compare it with state-of-the-arts (Starlink, OneWeb, Kuiper, \etc).}

	$$\sec R=\sqrt{3}\tan{\left(\frac{\pi}{6}\frac{N}{N-2}\right)}$$
\end{compactenum}

\paragraphb{Limitation:} Coverage only. No networking or ISL.
\fi

==> state-of-the-art.tex <==
%\subsection{Why Not Existing IP Addressing?}
\subsection{Fundamental Limits of IP for Space}
\label{sec:problem:state-of-the-art}

\todo{Go deeper beyond experiments. Show the fundamental limitations of {\em any} logic IP-based designs.}

\p{Can be much sharper, beyond the following ``fundamental limit''
\begin{compactitem}
\item {\bf Mega} constellation (NEW compared to existing work) $\rightarrow$ More satellites than terrestrial ``cells'' $\rightarrow$ No ``one-to-one'' mapping $\rightarrow$ Impossible for ``virtual node''-like solutions to map each satellite to an area;
\item Satellites gradually move and ``seams'' among satellites $\rightarrow$ Always exist cases where some users are out of coverage $\rightarrow$ logical IP change will still happen, even if the following ``impossible result'' does not hold
\end{compactitem}
\todo{Re-organize this section to integrate all these points.}
}

We investigate the fundamental limitations of directly applying the state-of-the-art IP address to space networking.
The goal is to maximize the network service availability.
Specifically, we ask if there exists a IP-based scheme that can guarantee the following properties are guaranteed {\em anywhere, anytime} for {\em any} mega constellations:
\begin{compactenum}
\item No static users' IP address will change anytime, anywhere; and 
\item No re-convergence of routing tables.
\end{compactenum}
To achieve property (1), such a scheme should guarantee that as a satellite leaves an area, the users in this area still retain the same IP subnet.
To achieve property (2), such a scheme should ensure that the network topology is also invariant of the satellite movement, thus no need to re-compute the routing tables.
Given the high relative movement between satellites and earth, static binding between a IP address/subnet and network node is clearly deemed impossible to achieve both goals.

To this end, we explore if the dynamic binding between satellites and IP address/subnets would help for all mega constellations. 
Such idea was first proposed in \cite{ekici2000datagram, ekici2001distributed}. 
In this scheme, Each logical location is embodied at any given time by a certain physical satellite. 
As a satellite disappears over the horizon, its corresponding position becomes represented by the next satellite passing overhead and the state information (IP address/subnet allocation, routing table, \etc) is transferred to it. 
So the identity of satellite is not permanently coupled with its logical location, which is taken over by the successor satellite in the same plane. 
The routing is performed basically by considering these logical locations as hops and a fix topology is formed. 
A routing decision is made based on this fixed virtual topology, and consequently, the network layer is isolated from the satellite constellation dynamics. 
%In this way, it is not necessary to consider the satellite movements.
In this way, the terrestrial users in every area retains the same IP subnet and address, and the routing tables remain unchanged.

While appealing, however, we prove that such dynamic binding would be only helpful for a limited set of constellations.
Its usefulness is decided by the following lemma:


%\fixme{The term ``logical IP'' does not seem a well-accepted term in SIGCOMM. Find a more precise term instead.}

%\paragraphb{Is it possible to optimize logical IP for space?}

%\paragraphb{Fundamental limitations of logical IP:}

\begin{lem}[Stability of classical logic IP in space]
A mega constellation can always retain invariant IP address and topology {\em if and only if} all its orbits are repeat ground track orbits.
\label{lem:repeat-orbit}
\yuanjie{So far this is a hypothesis based on Rose constellation, Geostationary satellites, and polar orbits. The sufficiency is straightforward, but the necessity is not. }
\end{lem}

Lemma \ref{lem:repeat-orbit} is proved in Appendix~\ref{proof:repeat-orbit}.
Note that in reality, most commercial mega constellations (Space Starlink, Amazon Kuiper, OneWeb, TeleSat, \etc) do {\em not} meet the conditions in Lemma~\ref{lem:repeat-orbit}.
It implies classical IP will suffer from frequent address change and rerouting in these constellations. 
From Lemma~\ref{lem:repeat-orbit}, we can immediately get an impossibility result:
\begin{thm}[Fundamental limitations of logical IP]
\label{thm:impossibility}
\todo{To be more rigorous. Intuitively this should be true.} No routing or subnet allocation schemes based on classical logic IP can always guarantee the following properties for any mega constellations anywhere, anytime:
\begin{compactenum}
\item No static users' IP address will change anytime, anywhere; and 
\item No re-convergence of routing tables.
\end{compactenum}
\end{thm}

\yuanjie{This result should hold even if the constellation itself can fully cover the earth. For some special constellations (such as repeat ground tracking orbits, polar orbits, and geostationary orbits), it is possible to guarantee these two requirements anywhere, anytime (which is exactly the concept of ``virtual nodes''). However, this may not hold in general, especially for commercial constellations like Starlink, OneWeb, \etc. The position of this work is a {\bf generic} addressing scheme, rather than for specific constellations.}

Theorem \ref{thm:impossibility} is proved in Appendix~\ref{proof:impossibility}.
The intuition is that, \todo{High relative motion among satellites and earth + earth rotation $\rightarrow$ For any area, there does not always exist a satellite that can (1) fully cover this area; and (2) it can be successfully connected to all other satellites serving the adjacent areas.}




==> statement.tex <==
\subsection{Problem Statement}
\label{sect:problem:statement}

This work aims at reliable extreme mobility management in 4G, 5G and beyond.
%We seek a solution that achieves significantly less network failures, verifiable conflict-free policies, and hopefully improved performance in extreme mobility.
We seek a solution with significantly less network failures, verifiable conflict-free policies, and negligible latency/signaling/spectral overhead. %in extreme mobility. %overhead of latency and spectral waste in extreme mobility. 
%The solution should satisfy three properties:
The solution should be reliable with dramatic wireless dynamics in extreme mobility, during which it may experience errors, delays, and failures in all phases of mobility management.
%critical signaling loss/errors, delayed feedback, and conflict-prone policies. 
\iffalse
\begin{compactitem}
\item {\bf Critical signaling loss/errors} 
\item {\bf Delayed/unreliable feedback}
\item {\bf Complex, conflict-prone policies}
\end{compactitem}
\fi
\iffalse
\begin{compactitem}
\item {\bf Excellent reliability} under signaling loss, delayed and unreliable channel feedback, and policy-based decisions in extreme mobility;
%with significantly less network failures, verifiable conflict-free policies, and hopefully improved performance in extreme mobility; %and improved delay/spectrum efficiency in extreme mobility.
\item {\bf Retain policy flexibility} for the network operators.
\item {\bf Backward compatibility} with existing OFDM-based designs and static/low-speed mobility, without hurting wireless data performance;
\end{compactitem}
\fi
The solution should be backward-compatible with existing OFDM-based 4G/5G (especially data transfer) in static and low mobility, %, without hurting wireless data performance.
and retain flexible policy for the operators.

%\yuanjie{Rephrase them to map to design components.}


==> use-case.tex <==
\subsection{``Killer'' Use Cases in Space}
\label{sec:back:case}

\todo{Refer to TLC paper [SIGCOMM'19]. 
Note we are {\bf NOT} proposing solutions for these specific use cases.
Instead, we use these cases to motivate the design goals in $\S$\ref{sec:problem}.}

\paragraphb{$\bullet$ Ubiquitous Internet access for developing areas:}

\paragraphb{$\bullet$ In-flight Internet access:} Check HotMobile'16 and WWW'18 papers. \yuanjie{Motivate the {\bf stability} with this example.}

\paragraphb{$\bullet$ In-orbit computing and content distribution:} \yuanjie{Use this case to motivate the universal addressing.}

%\todo{Any more? How about vehicular inter-networking or IoT?}
